On The Statistical Representation Properties Of The Perturb-Softmax And The Perturb-Argmax Probability Distributions

The Gumbel-Softmax probability distribution allows learning discrete tokens in generative learning, while the Gumbel-Argmax probability distribution is useful in learning discrete structures in discriminative learning. Despite the efforts invested in optimizing these probability models, their statistical properties are under-explored. In this work, we investigate their representation properties and determine for which families of parameters these probability distributions are complete, i.e., can represent any probability distribution, and minimal, i.e., can represent a probability distribution uniquely. We rely on convexity and differentiability to determine these statistical conditions and extend this framework to general probability models, such as Gaussian-Softmax and Gaussian-Argmax. We experimentally validate the qualities of these extensions, which enjoy a faster convergence rate. We conclude the analysis by identifying two sets of parameters that satisfy these assumptions and thus admit a complete and minimal representation. Our contribution is theoretical with supporting practical evaluation.

==> Gibbs_Gumbel_Normal.tex <==
\newpage
\section{Properties of random perturbation distribution models}\label{Gibbs_Gumbel_Normal}
In this section, we explore the properties of the expected perturbed maximizer $\E_{\gamma  \sim \mathcal{G} } \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]$ corresponding to various random perturbation distributions.

When the collection of i.i.d. random variables $\gamma = \{\gamma_y : y \in Y \}$ that follow a distribution with a smooth probability density function, Corollary \ref{derive_probability}  showed that the following holds:
\begin{equation}
    \frac{\partial}{\partial \theta}\E_{\gamma  \sim \mathcal{G}} \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]  = P_\gamma \left(\arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \} = y^{*} \right) 
\end{equation}

Denote by $G(t) = P(\gamma_y \leq t)$ the cumulative
distribution function of $\gamma_y$.
The independence of $\gamma_y$ across
$y\in Y$ implies that:
\begin{equation}\label{max_prob_cdf}
\begin{split}
P_{\gamma}(\max_{y\in Y} \{\theta_{y} +  \gamma_{y}\} \leq t ) 
      &= P_{\gamma} \left( \forall_{y\in Y}\{ \theta_{y} +  \gamma_{y} \} \leq t \right)\\ 
      &= P_{\gamma}(\forall_{y\in Y}\{\gamma_y  \} \leq t - \theta_{y} )\\
      &= \prod_{y\in Y}G(t - \theta_{y} )\\
\end{split}   
\end{equation}
\subsection{Gibbs distribution with Gumbel random variables}\label{Gibbs_dist}

We focus on the Gumbel distribution with zero mean, which is described by its double exponential cumulative distribution function 
\begin{equation} \label{eq:g_CFD}
    G(t) = P(\gamma(y) \leq t) = e^{-e^{-(t + c)}}, 
\end{equation}
and the probability density function
\begin{equation} \label{eq:g_pdf}
    g(t) = e^{-(t+e^{-t})} 
\end{equation}
where $c \approx 0.5772$ is the Euler-Mascheroni constant.

The following identity is known \cite{Tamir2016} and its proof is given here for completeness. \begin{equation}
     P_{\gamma \sim g} \left( y = \arg \max_{\hat y} \{ \theta_{\hat y} +  \gamma_{\hat y}\} \right) \propto e^{\theta_y}.
\end{equation}

\begin{theorem} \label{theorem_logpartitionsigma} 
 Let $\gamma = \{\gamma_y : y \in Y \}$ be a collection of i.i.d. Gumbel random
variables with cumulative distribution function $G(t)$ (Equation \ref{eq:g_CFD}). 
Denote the partition function $\sum_{y \in Y}e^{\theta_y}$ as $Z(\theta)$. Then, the random variable 
$\max_{y \in Y} \{\theta_{y} +  \gamma_{y}\}$ is distributed according to the Gumbel distribution whose mean is the log-partition
function, $log Z(\theta)$.
\end{theorem}

\begin{proof}

The Gumbel, Frechet, and Weibull distributions, used in extremal statistics, are max-stable distributions: the product 
$\prod_{y \in Y}G(t - \theta_{y})$ can be described in terms of G(·) itself. Under the said setting,
the double exponential form of the Gumbel distribution yields the result:
\begin{equation}
\begin{split}
\prod_{y \in Y}G(t - \theta_{y}) &= e^{- \sum_{y\in Y}e^{- (t - \theta_{y} + c )}} \\
 &= e^{- e^{- (t + c - \log Z(\theta) )}} \\
 &= G(t-\log Z(\theta)
\end{split}   
\end{equation}  
The proof concludes by the identity in Equation \ref{max_prob_cdf}. 
\end{proof}

Under these conditions, it holds for all $y$:
\begin{equation*}
\frac{e^{\theta_y}}{Z(\theta)} = P_{\gamma}(y = \arg \max_{\hat y \in Y} \{\theta_{\hat y}+ \gamma_{\hat y}\})
\end{equation*} 

\begin{proof}
For Gumbel random
variables with cumulative distribution function $G(t) $(Equation \ref{eq:g_CFD}) it holds:
\begin{equation} \label{GumbelProperty}
G'(t)  = e^{-t}G(t) 
 = e^{-t}e^{- e^{-t}} 
 = e^{-t-e^{-t}}
 = e^{-(t+e^{-t})} 
 = g(t).
\end{equation}

Putting it together we have that:
$\mathbb{E}_{\gamma}\left( \max_{y \in Y} \{\theta_y+\gamma_y\} \right) = \log Z(\theta)$ (Theorem \ref{theorem_logpartitionsigma}). 
We can derive w.r.t. some $\theta_{y'}$.
We note that by differentiating the right-hand side we get:
\begin{equation}
\begin{split}
\frac{\partial \log Z(\theta)}{\partial \theta_{y'}} 
&= \frac{e^{\theta_{y'}}}{ Z(\theta)}
\end{split}
\end{equation}
Differentiate the left-hand side:
First, we can differentiate under the integral sign:
\begin{equation*}
\frac{\partial}{\partial \theta_{y'}} \int_{\rm I\!R^{|Y|}} \max_{y \in Y} \{\theta_y+\gamma_y\} d\gamma
=  \int_{\rm I\!R^{|Y|}}\frac{\partial}{\partial \theta_{y'}} \max_{y \in Y} \{\theta_y+\gamma_y\} d\gamma
\end{equation*}  
We can write a subgradient of the max-function using an
indicator function (an application of Danskin’s Theorem \cite{bertsekas2003convex}):
\begin{equation*}
\frac{\partial}{\partial \theta_{y'} }max_{y \in Y} \{\theta_y+\gamma_y\} = \mathds{1}(y' = \arg \max_{y \in Y} \{\theta_y+\gamma_y\})  
\end{equation*}  
The corollary then follows by applying the expectation to both
sides of the last equation.
\end{proof}

An alternative proof of the preceding argument can also be made.

\begin{eqnarray}
P_{\gamma}(y' = \arg \max_{y \in Y} \{\theta_y+\gamma_y\} ) &=& \int_{t} g(t -\theta_{y'}) \prod_{y \neq y'} G(t-\theta_{y})dt\\
    \star &=& \int_{t} G' (t -\theta_{y'}) \prod_{y \neq y'} G(t-\theta_{y})dt \\
    \star \star &=& \int_{t} e^{-(t- \theta_{y'})}G(t-\theta_{y'})\prod_{y \neq y'} G(t-\theta_{y})dt \\
    &=& e^{\theta_{y'}} \int_{t} e^{-t}\prod_{y} G(t-\theta_{y})dt\\
    &=& e^{\theta_{y'}}*constant
\end{eqnarray}


Therefore the probability that $y'$ maximizes $\theta_y+\gamma_y$ is proportional to
$ e^{\theta_{y'}}$.

$\star$ and $\star\star$ are due to the probability density function of the Gumbel distribution as shown in Equation \ref{GumbelProperty}.


\subsection{Normal random variables}\label{Gaussian_randomvariables}

Equation \ref{max_prob_cdf} showed that the following holds:
\begin{equation}
P_{\gamma}(\max_{y\in Y} \{\theta_{y} +  \gamma_{y}\} \leq t ) =  \prod_{y\in Y}G(t - \theta_{y} )
\end{equation}

Consider now a collection of independent random variables $\gamma = \{ \gamma_y : y \in \mathcal{Y} \}$ that follow the Normal distribution, $\gamma_y \sim \mathcal{N}(\theta_y,1)$, which is described by its cumulative distribution function 
\begin{equation}
    G(t-\theta_y) = \frac{1}{\sqrt{2\pi}} \int_{-\infty}^{t}e^{-\frac{(t-\theta_y)^2}{2}} dt \label{cdf_theta}, 
\end{equation}
and the probability density function
\begin{equation}
    g(t-\theta_y) = \frac{1}{\sqrt{2\pi}} e^{-\frac{(t-\theta_y)^2}{2}}. 
\end{equation}

\paragraph{The error function, the complementary error function and CDF} The related error function $\operatorname {erf(t)}$ gives the probability of a random variable, with normal distribution of mean 0 and variance 1/2 falling in the range $[-t,t]$. That is:
\begin{equation}
    \operatorname {erf(t)}={\frac {2}{\sqrt {\pi }}}\int _{0}^{t}e^{-x^{2}}\,dx
\end{equation}
and the complementary error function is defined as
\begin{eqnarray}
    \operatorname {erfc(t)} &=& {\frac {2}{\sqrt {\pi}}}
    \int _{t}^{\infty} e^{-x^{2}}\,dx \\
    &=& 1 - \operatorname {erf(t)}.
\end{eqnarray}
The CDF of the standard normal distribution can be expressed with its error function and complementary error function 
\begin{eqnarray}
    G(t) &=& {\frac {1}{2}}\left(1+\operatorname {erf} \left({\frac {t}{\sqrt {2}}}\right)\right)  \label{cdf_erf}.\\
    &=& {\frac {1}{2}}\operatorname {erfc} \left({\frac {-t}{\sqrt {2}}}\right) \label{cdf_erfc}.
\end{eqnarray}
The last identity holds since $\operatorname {-erf(t)} = \operatorname {erf(-t)}$, hence $1-\operatorname {erf} \left({\frac {t}{\sqrt {2}}}\right)= 1+\operatorname {erf} \left({\frac {-t}{\sqrt {2}}}\right)$.

Therefore, expressing $G(t-\theta_y)$ (Equation \ref{cdf_theta}) in terms of its error function, as done for the standard normal distribution in Equation \ref{cdf_erf}, shows that 
\begin{equation}
    G(t-\theta_y) = {\frac {1}{2}}\left(1+\operatorname {erf} \left({\frac {t-\theta_y}{\sqrt {2}}}\right)\right)  \label{cdf_theta_erf}.
\end{equation}
Therefore 
\begin{eqnarray}
    P_{\gamma}(\max_{y\in Y} \{\theta_{y} +  \gamma_{y}\} \leq t ) &=& \prod_{y\in Y}G(t - \theta_{y} ) \\
    &=&  \prod_{y\in Y}{\frac {1}{2}}\left(1+\operatorname {erf} \left({\frac {t-\theta_y}{\sqrt {2}}}\right)\right).
\end{eqnarray}

Furthermore, the probability that $y'$ maximizes $\theta_y+\gamma_y$ is
\begin{eqnarray}
    P_{\gamma}(y' = \arg \max_{y \in Y} \{\theta_y+\gamma_y\} ) &=& \int_{t} g(t -\theta_{y'}) \prod_{y \neq y'} G(t-\theta_{y})dt\\
    &=& \frac{1}{\sqrt{2\pi}} e^{-\frac{(t-\theta_{y'})^2}{2}} \prod_{y \neq y'}{\frac {1}{2}}\left(1+\operatorname {erf} \left({\frac {t-\theta_y}{\sqrt {2}}}\right)\right).
\end{eqnarray}    
\iffalse
\textcolor{blue}{
A useful asymptotic expansion of the complementary error function (and therefore also of the error function) for large real t, $\operatorname {erfc(t)}  \approx \frac{e^{-t^2}}{\sqrt {\pi}t}$.
Then, this asymptotic expansion on Equation \ref{cdf_erfc}, 
\begin{equation}
    \ln G(t) \approx  -\frac{e^{-t^2/2}}{\sqrt {2\pi}t}
\end{equation}
Then,
\begin{equation}
    \ln G(t)^{n}=n\ln G(t) \approx -{\frac {ne^{-t^{2}/2}}{{\sqrt {2\pi }}t}}.
\end{equation}
Thus we have
\begin{equation}
    G(t)^{n}\approx e^{ -{\frac {ne^{-t^{2}/2}}{{\sqrt {2\pi }}t}}}.
\end{equation}
}
\fi

\iffalse
\subsubsection*{blackboard log-sum-exp}
Define $z(\theta) = \log (\sum_{y \in Y} \exp^{\theta_y})$.
Then, its convex conjugate is
\begin{equation}
    z^{*}\left(\theta^{*}\right):=\max _{\theta}\{\langle \theta^{*},\theta\rangle -\log \sum_{\hat y \in Y} \exp^{\theta_{\hat y}}\}
\end{equation}

Derivative w.r.t. $\theta_y$
\begin{eqnarray}
    \frac{\partial}{\partial \theta_y} \left( \langle \theta^{*},\theta\rangle -\log \sum_{\hat y \in Y}\exp^{\theta_{\hat y}} \right) &=& 0\\
    \theta^{*}_y &=& \frac{\exp^{\theta_y} }{\sum_{\hat y \in Y} \exp^{\theta_{\hat y}} }
\end{eqnarray}
denote $\theta^{*}_y $ by $p_y$.
Then, the convex conjugate, which is the negative Shannon entropy.
\begin{eqnarray}
    z^{*}\left(\theta^{*}\right) &=& \sum_{y \in \mathcal{Y}}\theta_y p_y - \log \sum_{y \in Y}\exp^{\theta_y} \\
    &=& \sum_{y \in \mathcal{Y}} p_y(\theta_y- \log \sum_{y \in Y}\exp^{\theta_y} )\\
    &=& \sum_{y \in \mathcal{Y}} p_y(\log \exp^{\theta_y}- \log \sum_{y \in Y}\exp^{\theta_y} )\\
    &=& \sum_{y \in \mathcal{Y}} p_y log p_y
\end{eqnarray}
\fi

==> PerturbedMaximizers.tex <==

\begin{definition}\label{def:essentially-smooth-function}
    An essentially smooth function.
    A convex function $f$ is essentially smooth if it has a nonempty domain $C = dom(f)$, $f$ is differentiable throughout $C$, and $\lim_{i\rightarrow \infty} \nabla f(x_i) =+ \infty$ for any sequence $\{x_i\}$ contained in $C$, and converging to a boundary point of $C$. A convex function with domain $\R^d$ is always essentially smooth since its domain has no boundary.
\end{definition}

\begin{definition}
\label{def:continuous-functions} Properties of continuous functions. 
If $f:{\mathbb  {R}}^{d}\rightarrow {\mathbb  {R}}$ is a continuous function and
${\mbox{dom}}f$ is closed, then $f$ is closed.
If $f:{\mathbb  {R}}^{d}\rightarrow {\mathbb  {R}}$ is a continuous function and
${\mbox{dom}}f$ is open, then $f$ is closed if and only if it converges to $\infty$  along every sequence converging to a boundary point of ${\mbox{dom}}f$.
\end{definition}

\begin{definition}\label{def:proper-convex- function}
A proper convex function.
If $f$ is a convex function or if a minimum point of $f$ is being sought, then $f$ is called proper if  $f(x)> -\infty$ for every $x \in dom f$
and if there also exists some point
$x_{0}$ in its domain such that
${\displaystyle f\left(x_{0}\right)<+\infty }$. Meaning that a function is proper if its effective domain is nonempty and it never attains the value $-\infty$.
\end{definition}

\begin{definition}
The domain of the convex conjugate $f^*$ is \begin{equation}\label{definition:domain}
        domf^* = \{\lambda : \sup_{\theta} \{\langle \lambda,\theta \rangle - f(\theta)\} <\infty \}.
    \end{equation}  
\end{definition}

\begin{definition}\label{def:highdim_convexity}
    A function $g: \R^n \rightarrow \R$
is convex if and only if the function $h: \R \rightarrow \R$ given
by $h(t) = g(x + tv)$ is convex (as a univariate function) for all $x$ in domain of $g$ and all
$v \in  \R^n$.
\end{definition}

\begin{definition}\label{def:single_valued_function}
A single-valued function is function that, for each point in the domain, has a unique value in the range. It is therefore one-to-one or many-to-one.
\end{definition}

\begin{definition}\label{def:minimal_representation}
    An exponential family is referred to as minimal if there are no linear constraints among the components of the parameter vector nor are there linear constraints among the components of the sufficient statistic (in the latter case, with probability
one under the measure $\mu$), i.e. there is no set of coefficients $\alpha \in \R^s, \alpha \neq 0$
such that,
$\sum_{j=1}^{s}\alpha_j \theta^j = const$.
\end{definition}

\begin{definition}
$f^*$ is the convex conjugate of the function $f$. That is,
\begin{equation}
    f^{*}\left(\lambda\right):=\sup _{x\in dom(f)}\{\left.\left\langle \lambda,x\right\rangle -f\left(x\right)\right \}
\end{equation}
\end{definition}

\section{Perturbed Maximizers}
\label{PerturbedMaximizers}


For $\theta \in \R^d$, and for i.i.d. random variables $\gamma \in \R^d$ that follow distribution $\mathcal{G}$ with a smooth probability density function $q$, let 
\begin{equation}
f(\theta) = \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]
\end{equation} 
denote the expected perturbed maximum over the domain $\mathcal{C} =\R^d$. Let $f(\theta)$ take values over the extended real domain $\R \cup \{\pm \infty\}$.

Note that our notation $\max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\}$ is equivalent to $ \max_{y \in \mathcal{Y}}\{ \langle y, \theta+ \gamma \rangle \}$.


\begin{theorem}\label{theorem1}
   There is a single-valued mapping between $\E_{\gamma  \sim \mathcal{G} } \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]$ and 
   $P_\gamma \left( \arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \} = y^{*} \right)$.
\end{theorem}
\begin{proof}
$f(\theta)$ is a closed proper convex function and is also essentially smooth as the following conditions hold:
 \begin{enumerate}
     \item By Corollary \ref{convexity}, $f(\theta)$ is convex.
     \item $f(\theta)$ is proper.
     \item By Corollary \ref{max_differtiable}, $f(\theta)$ is infinitely differentiable throughout the domain $\mathcal{C}$, therefore it is a smooth function throughout its domain. 
    \item $f(\theta)$ is a smooth convex function on $R^d$, therefore it is in particular essentially smooth. 
    \item The smoothness of  $f(\theta)$ guarantees its continuity, and since $R^d$ can be considered a closed set,  then $f(\theta)$ is a closed function.
 \end{enumerate}
The proof concludes by Corollary \ref{derive_probability}, which showed that $\frac{\partial}{\partial \theta}\E_{\gamma  \sim \mathcal{G}} \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]  = P_\gamma\left( \arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \}) = y^{*} \right)$ per Theorem 26.1 in \cite{rockafellar-1970a}.
\end{proof}

\begin{corollary}\label{convexity}
    $f(\theta)$ is a convex function.
\end{corollary}
\begin{proof}

$f(\theta)$ is convex as a maximum of convex (linear) functions. 
\end{proof}

\begin{corollary}\label{derive_probability}

   
\begin{equation}
    \frac{\partial}{\partial \theta}\E_{\gamma  \sim \mathcal{G}} \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right] = P_\gamma \left( \arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \} = y^{*} \right)
\end{equation} 
\end{corollary}

\begin{proof}
First, we can differentiate under the integral:
\begin{equation}
    \frac{\partial}{\partial\theta}  \int q(\gamma) \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} d\gamma = \int q(\gamma) \frac{\partial}{\partial\theta} \max_{y \in \mathcal{Y}} \{\theta_y+ \gamma_y\} d\gamma
\end{equation}  
We can write a subgradient of the max-function using an
indicator function (an application of Danskin’s Theorem):
\begin{equation}
    \frac{\partial}{\partial\theta} \max_{y \in \mathcal{Y}} \{\theta_y+ \gamma_y\} = \mathds{1}_{\arg \max_{y \in \mathcal{Y}} \{\theta_y+ \gamma_y\} = y^*} 
\end{equation}  
The corollary then follows by applying the expectation to both
sides of the last equation.
\begin{eqnarray}
    \frac{\partial}{\partial \theta}\E_{\gamma  \sim \mathcal{G}} \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right]  &=& \E_{\gamma  \sim \mathcal{G}} \left[ \mathds{1}_{\arg \max_{y \in \mathcal{Y}} \{\theta_y+ \gamma_y\} = y^*} \right] \\
    &=& P_\gamma \left(\arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \} = y^{*} \right) \label{perturbedmaximizerprob}
\end{eqnarray}
\end{proof}

\begin{corollary}\label{max_differtiable}
    The expected perturbed maximum, $ f(\theta)$, is differentiable throughout the domain $\mathcal{C}$.
\end{corollary}

\begin{proof}
    
\begin{eqnarray}
    \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y \in \mathcal{Y}}\{ \theta_y+ \gamma_y\} \right] &=& \E_{\gamma  \sim \mathcal{G}} \left[ \mathds{1}_{\arg \max_{y \in \mathcal{Y}} \{\theta_y+ \gamma_y\} = y^*} \right] \\
    &=& \int q(\gamma) \mathds{1}_{\arg \max _{y \in \mathcal{Y}} \{ \theta_y+ \gamma_y \} = y^{*}} d \gamma 
\end{eqnarray} 
A change of variables
\begin{eqnarray}
    \bar{\gamma}= \theta + \gamma
\end{eqnarray}
then,
\begin{equation}
    \E_{\gamma \sim \mathcal{G} } \left[ \max_{y \in \mathcal{Y}}\{ \theta_y + \gamma_y\} \right] = \int q(\bar{\gamma} - \theta) \mathds{1}_{\arg \max _{y \in \mathcal{Y}} \{ \bar{\gamma} \}= y^*}d \bar{\gamma}. \label{expectedmax_deltadirac}
\end{equation}

With this formulation, it is evident that $f(\theta)$ is infinitely differentiable in the domain $\mathcal{C}$ with respect to $\theta$, since $\theta$ is only incorporated in the smooth function $q$.
Hence, the expected perturbed maximum is a smooth function w.r.t. $\theta$. 
\end{proof}


\subsection{The convex conjugate of the expected perturbed maximum}

Define $f(\theta) =\E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right]$ with domain $\R^d$. $\gamma \in \R^d$ are i.i.d. random variables that follow distribution $\mathcal{G}$ with a smooth probability density function $q$. Let $f(\theta)$ take values over the extended real domain $\R \cup \{\pm \infty\}$,  $f(\theta):\R^d \rightarrow \R \cup \{\pm \infty\} $.
Then, its convex conjugate is

\begin{equation}
    f^{*}\left(\lambda\right):=\sup _{\theta} \{\langle \theta,\lambda \rangle - \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right]\}
\end{equation}

Its derivative w.r.t. $\theta_y$
\begin{eqnarray}
    \frac{\partial}{\partial \theta_y} \left( \langle \theta,\lambda \rangle - \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right] \right) &=& 0 \\
    \lambda^{*}_y = P_\gamma \left(y= \arg \max _{\hat y} \{ \theta_{\hat y}+ \gamma_{\hat y} \}  \right) \label{expectedmaximizer_probabilities}.
\end{eqnarray}

Then, the convex conjugate for $\lambda^{*}_y $, denoted by $p_y$, is
\begin{eqnarray}
   f^{*}\left(\lambda\right) &=&  \sum_{y}\theta_y p_y - \E_{\gamma} \left[ \left(\sum_{\hat y \in \mathcal{Y}} \mathds{1}_{\arg \max _{y \in \mathcal{Y}} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \right)   \max _{y \in \mathcal{Y}} \{  \theta_{y}+ \gamma_{y}\} \right] \\
   &=&  \sum_{y}\theta_y p_y - \sum_{\hat y} \E_{\gamma } \left[ \mathds{1}_{\arg \max _{y} \{  \theta_{y}+ \gamma_{y} \} = \hat y} \max _{y} \{ \theta_{y}+ \gamma_{y} \} \right] \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y } \E_{\gamma } \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y} \} = \hat y}  (\theta_{\hat y}+ \gamma_{\hat y}) \right] \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{\theta_{y}+ \gamma_{y} \} = \hat y}  \theta_{\hat y} \right] -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y} \} = \hat y} \gamma_{\hat y} \right]  \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y } p_{\hat y} \theta_{\hat y}  -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \gamma_{\hat y} \right] \\
     &=&   -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \gamma_{\hat y} \right] \\
     &=&  -\sum_{\hat y} p_{\hat y} \E_{\gamma} \left[ \gamma_{\hat y} \right] \\
      &=&   -\E_{\gamma} \left[ \gamma_{y^*} \right] 
\end{eqnarray}

where $ \gamma_{y^*}$ denotes $\gamma_y$ for which $\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = y^*$.

Therefore, the convex conjugate of $f(\theta)$ takes the following values
\begin{equation}\label{conjugate_cases_max}
    f^{*}\left(\lambda\right) =
        \begin{cases}
            -\E_{\gamma} \left[ \gamma_{y^*} \right] &\quad\text{if } \lambda = \lambda^{*}\\
            \infty &\quad\text{otherwise}
        \end{cases}
\end{equation}


\iffalse
\subsubsection*{blackboard expected perturbed maximum}

Define $z(\theta) =\E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right]$.
Then, the convex conjugate $z^*(\theta)$

\begin{equation}
    z^{*}\left(\theta^{*}\right):=\max _{\theta}\{\langle \theta^{*},\theta\rangle - \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right]\}
\end{equation}

Derivative w.r.t. $\theta_y$
\begin{eqnarray}
    \frac{\partial}{\partial \theta_y} \left( \langle \theta^{*},\theta\rangle - \E_{\gamma  \sim \mathcal{G} } \left[ \max_{y}\{ \theta_y+ \gamma_y \} \right] \right) &=& 0 \\
    \theta^{*}_y = P \left(y= \arg \max _{\hat y} \{ \theta_{\hat y}+ \gamma_{\hat y} \}  \right)
\end{eqnarray}

denote $\theta^{*}_y $ by $p_y$.
Then, the convex conjugate 
\begin{eqnarray}
   z^{*}\left(\theta^{*}\right) &=&  \sum_{y}\theta_y p_y - \E_{\gamma} \left[ \left(\sum_{\hat y} \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \right)   \max _{y} \{  \theta_{y}+ \gamma_{y}\} \right] \\
   &=&  \sum_{y}\theta_y p_y - \sum_{\hat y} \E_{\gamma } \left[ \mathds{1}_{\arg \max _{y} \{  \theta_{y}+ \gamma_{y} \} = \hat y}  \max _{y} \{ \theta_{y}+ \gamma_{y} \} \right] \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y } \E_{\gamma } \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y} \} = \hat y}  (\theta_{\hat y}+ \gamma_{\hat y}) \right] \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{\theta_{y}+ \gamma_{y} \} = \hat y}  \theta_{\hat y} \right] -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y} \} = \hat y} \gamma_{\hat y} \right] 
    \nonumber \\
    &=&  \sum_{y}\theta_y p_y - \sum_{\hat y } p_{\hat y} \theta_{\hat y}  -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \gamma_{\hat y} \right] \\
     &=&   -\sum_{\hat y} \E_{\gamma} \left[ \mathds{1}_{\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = \hat y}  \gamma_{\hat y} \right] \\
     &=&  -\sum_{\hat y} p_{\hat y} \E_{\gamma} \left[ \gamma_{\hat y} \right] \\
      &=&   -\E_{\gamma} \left[ \gamma_{y^*} \right] \\
\end{eqnarray}

where $ \gamma_{y^*}$ denotes $\gamma_y$ for which $\arg \max _{y} \{ \theta_{y}+ \gamma_{y}  \} = y^*$
\fi 


    
\begin{theorem}\label{theorem_unbounded_smooth_perturb}
The range of the probabilities of the perturbed maximizer (maximizing argument) (Equation \ref{perturbedmaximizerprob}) differs very little from the probability simplex, denoted $\Delta$, such that 
\begin{equation}
    ri( \Delta) \subseteq \text{range } \partial f \subseteq \Delta.
\end{equation}
\end{theorem}
\begin{proof}
    
Recall that the derivative of the expected perturbed maximum  $f(\theta)$ is the probability of the expected maximizer (Equation \ref{perturbedmaximizerprob}).  $f(\theta)$ is a closed proper convex function on $R^d$ (Theorem \ref{PerturbedMaximizers}), then per Corollary 23.5.1 and (beginning of chapter 24) \cite{rockafellar-1970a} the following holds for 
the range of $\partial f $:
\begin{equation}\label{rockafellar_rangedf}
   ri( dom f^*) \subset \text{range } \partial f \subset dom f^*,
\end{equation}
    where 
    \begin{equation}
        \text{range }  \partial f  = \cup \{ \partial f(\theta) | \theta \in R^n \}.
    \end{equation}

The proof follows two steps:
that $ \text{range }  \partial f \subseteq \Delta$ and that $ri (\Delta) \subseteq  ri (dom f^*)$.

First, it holds that $domf^* \subseteq \Delta$, since 
$domf^* \subseteq \{\lambda \in \R^d: \sum_{y} \lambda_y=1, \lambda_y \geq 0 \;  \forall \lambda_y\}$ (Equations \ref{expectedmaximizer_probabilities}, and \ref{conjugate_cases_max}). Since  $ \text{range } \partial f \subset dom f^*$   (Equation \ref{rockafellar_rangedf}, it holds also that  $\text{range }  \partial f  \subseteq \Delta$.

Next, we prove that $ri(\Delta)\subseteq  ri (dom f^*)$. Consider $\theta_n^i = (0,\dots, n ,\dots,0)$, $\theta_n^i \in \R^d$, a vector of all zeros, except its value in the $i^{th}$ position is $n$. Then, it holds that $\partial f(\theta^i_n)  \in \Delta$ and also $\partial f(\theta^i_n) \in dom f^*$, since we proved that $\text{range } \partial f \subset dom f^* \subseteq \Delta$. Moreover, it holds that $\cup_{1 \leq i \leq d, n\in \mathcal{N}} \partial f(\theta^i_n) \subseteq \text{range } \partial f $. 

The sequence $\left( \partial f(\theta^i_n)\right)_{n_0}^{\infty}$ is a monotonic and bounded sequence of real numbers, then by the monotone convergence theorem its limit exists.
Hence, the derivative of the perturbed maximizer $f(\theta^i_n)$ approaches an extreme point of the probability simplex as $n \rightarrow \infty$, since
\begin{eqnarray}\label{limit_prob}
    \lim_{n \rightarrow \infty} \partial f(\theta^i_n) &=& \lim_{n \rightarrow \infty} (\frac{\partial f(\theta^i_n)}{\partial \theta^1},\dots, \frac{\partial f(\theta^i_n)}{\partial \theta^i},\dots, \frac{\partial f(\theta^i_n)}{\partial \theta^d}) \nonumber  \\ 
    &=& (0,\dots, 1, \dots,0) . 
\end{eqnarray}
Therefore, it holds that it is a point in the closure of the $dom  f^*$, $\lim_{n \rightarrow \infty} \partial f(\theta^i_n) \in cl(dom  f^*)$.
The domain of the convex conjugate $\text{dom } f^*$ is a convex set \cite{rockafellar-1970a}, Theorem 3.4)\iffalse (\textcolor{purple}{facts 1,3 below})\fi. Its convexity assures that following the line segment principle (\textcolor{purple}{fact 4 below}), all points on the line segment connecting $\partial f(\theta^i_n) \in ri(dom  f^*)$ and $\lim_{n \rightarrow \infty} \partial f(\theta^i_n) \in cl(dom  f^*) $, except possibly
$\lim_{n \rightarrow \infty} \partial f(\theta^i_n)$, belong to relative interior of $dom  f^*$.  
Assume by contradiction that $\lim_{n \rightarrow \infty} \partial f(\theta^i_n)$ does not belong to the relative interior of $dom  f^*$. Then, by separation axiom $T_0$, it holds that given the point $\lim_{n \rightarrow \infty} \partial f(\theta^i_n)$ and a point $\partial f(\theta^i_{n'}) \in ri(dom  f^*)$, at least one of them has an open neighborhood not containing the other point. However, since $n'$ can be arbitrarily large, point $\partial f(\theta^i_{n'})$ can be arbitrarily close to point $\lim_{n \rightarrow \infty} \partial f(\theta^i_n)$, such that the open neighborhood of point $\partial f(\theta^i_{n'})$ must include the extreme point $\lim_{n \rightarrow \infty} \partial f(\theta^i_n)$ and vice versa. We conclude that the extreme point of the probability simplex 
$\lim_{n \rightarrow \infty} \partial f(\theta^i_n) \in  ri (dom f^*)$ .
Then, as $n \rightarrow \infty $, $\Delta$ and $dom f^*$ have the same relative interior (and hence
the same closure (\textcolor{purple}{fact 5 below})), meaning $ri(\Delta) \subseteq ri (dom f^*)$.

Therefore, the range of the probabilities of the perturbed maximizer (maximizing argument) differs very little from the probability simplex. 
\end{proof}


\paragraph{other facts}
\begin{enumerate}
    \item Let $f$ be a function whose values are real or $\pm \infty$ and whose domain is in a subset $S$ of $\R^n$. The set  
    \begin{equation}
        \{(x,\mu) | x \in S, \mu \in \R, \mu \geq f(x) \}
    \end{equation}
    is called the epigraph of $f$ and is denoted by $epi(f)$. The effective domain of a convex function $f$ on $S$, $dom f$, is the projection on $\R^n$ of the epigraph of f:
    \begin{equation}
        dom f  = \{x |\exists\mu, (x,\mu)\in epi f \}= \{x|f(x) < +\infty \}.
    \end{equation}
    Then, $dom f $ is a convex set in $\R^d$, since it is the image of the convex set $epi f$ under linear transformation (Theorem 3.4, page 23 \cite{rockafellar-1970a} ).
    \item Theorem 12.2 : Let $f$ be a convex function. Then, its convex conjugate $f^*$ is a closed convex function, proper if and only if $f$ is proper.
    Also, the convex conjugate $f^*$ is a convex function, even if $f$ is not convex.
    \item The relative interior of a convex set in $R^d$ is also convex (Theorem 6.1, 6.2 \cite{rockafellar-1970a}).
    \item The line segment principle: If $C$ is a convex set, $x \in ri(C)$ and $\bar x \in cl(C)$, then all points on the line segment connecting $x$ and $\bar x$, except possibly
    $\bar x$, belong to $ri(C)$.
    \item Let $C$ be a nonempty convex set. Let $\bar C$ be another nonempty convex set. The following three conditions are equivalent:
    (i) $C$  and $\bar C$ have the same relative interior.
    (ii) $C$  and $\bar C$ have the same closure.
    (iii) $ri(C) \subset  \bar C \subset cl(C) $.
\end{enumerate}


\paragraph{The separation axioms}

\href{https://ncatlab.org/nlab/show/separation+axioms}{separation axioms}
\begin{enumerate}
    \item The $T_0$ (Kolmogorov) separation axiom: Given two distinct points, at least one of them has an open neighborhood not containing the other point.
    \item The $T_1$ separation axiom: Given two distinct points, both have an open neighborhood not containing the other point.
    \item The $T_2$ (Hausdorff) separation axiom: Given two distinct points, they have disjoint open neighborhoods.
    \item The $T_3$ (regular Hausdorff) separation axiom: $T_1$ and given a point and a closed subset not containing it, they have disjoint open neighborhoods.
    \item The $T_4$ (normal Hausdorff) separation axiom: $T_1$ and given two disjoint closed subsets, they have disjoint open neighborhoods.
\end{enumerate}

\begin{definition} Neighborhood. In topology, a neighborhood of a point 
$x$ in some topological space $X$ is a subset $U$ such that there is enough room around $x$ in $U$ to move in any direction (but perhaps not very far). One writes $x \in U^o$, or any of the other variations to indicate that $U$ is a neighborhood of $x$.
\end{definition}

Let $(X,\tau)$ be a topological space and $x \in X$ a point. Then:
\begin{enumerate}
    \item A subset $U \subset X $ is a neighbourhood of $x$ if there exists an open subset $O \subset X $ such that $x \in O$ and $O \subset U$.
    \item A subset $U \subset X $ is an open neighbourhood of $x$ if it is both an open subset and a neighbourhood of $x$.
\end{enumerate}



\subsection{The expected perturbed maximum for discrete random variable perturbations}\label{expectedmax_discretechapter}

For $\theta \in \R^2$, and for i.i.d. random variables $\gamma \in \{1,-1\}$, such that $P(\gamma = 1)=P(\gamma=-1)=\frac{1}{2}$. Let $f(\theta) = \E_{\gamma } \left[ \max_{i}\{ \theta_i+ \gamma_i\} \right]$ denote the expected perturbed maximum over the domain $\mathcal{C} =\R^d$. Let $f(\theta)$ take values over the extended real domain $\R \cup \{\pm \infty\}$. Clearly, $P(1= \arg \max_i \{\theta_i+\gamma_i \}) = P(\theta_1+\gamma_1 \geq \theta_2+\gamma_2)$.

\begin{eqnarray}
    f(\theta) &=& \E_{\gamma } \left[ \max_i\{ \theta_i+ \gamma_i\} \right] \\
    &=& P(\gamma_1=1,\gamma_2 =1)\left(1+ \max\{\theta_1,\theta_2\}\right) + P(\gamma_1=-1,\gamma_2 =-1)\left(\max\{\theta_1, \theta_2\}-1\right) \\
    &+& P(\gamma_1=1,\gamma_2 =-1)\left(
    \max\{\theta_1+1, \theta_2-1\}\right) +P(\gamma_1=-1,\gamma_2 =1)\left(\max\{\theta_1-1, \theta_2+1\}\right) \nonumber \\   
    &=& \frac{1}{2}\left(\max\{\theta_1, \theta_2\}\right)
    + P(\gamma_1=1,\gamma_2 =-1)\left(
    \max\{\theta_1+1, \theta_2-1\}\right) +P(\gamma_1=-1,\gamma_2 =1)\left(\max\{\theta_1-1, \theta_2+1\}\right) \\
    &=& \frac{1}{2}\left(\max\{\theta_1, \theta_2\}\right)
    + \frac{1}{2}\left(\frac{\max\{\theta_1+1, \theta_2-1\}}{2}+\frac{\max\{\theta_1-1, \theta_2+1\}}{2}\right) \label{max_discrete_f}
\end{eqnarray}

Equation \ref{max_discrete_f} suggests the following ranges of $f(\theta)$:

\begin{figure}[ht]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/discrete_ranges.jpg}
  \label{fig:sub1}
\end{subfigure}
\caption{Maximum ranges of $f(\theta)$.}
\label{fig:discrete_max_ranges}
\end{figure}


\begin{equation}\label{discrete_max_ranges}
    f(\theta) =
        \begin{cases}
        \theta_1 &\quad\text{if } \theta_1 \geq \theta_2+2\\

        \frac{3}{4}\theta_1  + \frac{1}{4}\theta_2+ \frac{1}{2} &\quad\text{if }  \theta_2+2 \geq \theta_1 \geq \theta_2\\

        \frac{3}{4}\theta_2  + \frac{1}{4}\theta_1+ \frac{1}{2} &\quad\text{if }\theta_2-2 \leq  \theta_1 \leq  \theta_2\\
        
        \theta_2 &\quad\text{if } \theta_1 \leq \theta_2-2
        \end{cases}
\end{equation}


Note that the following indeed holds:
\begin{equation}
    f(\theta) =
        \begin{cases}
         \theta_1  =  \frac{3}{4}\theta_1  + \frac{1}{4}\theta_2+ \frac{1}{2}& \quad\text{if } \theta_1 =  \theta_2+2\\

        \frac{3}{4}\theta_1  + \frac{1}{4}\theta_2+ \frac{1}{2} =  \frac{3}{4}\theta_2  + \frac{1}{4}\theta_1+ \frac{1}{2} &\quad\text{if }  \theta_1 = \theta_2\\

        
        \theta_2 =\frac{3}{4}\theta_2  + \frac{1}{4}\theta_1+ \frac{1}{2} &\quad\text{if } \theta_1 = \theta_2-2
        \end{cases}
\end{equation}

\subsubsection{The derivative of the perturbed expected max }
The derivative of $\frac{\partial}{\partial \theta}f(\theta) = (\frac{\partial}{\partial \theta_1}f(\theta), \frac{\partial}{\partial \theta_2}f(\theta))$ corresponds to the probabilities of the arg max $(P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 1 \right),P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 2 \right))$  (Equation \ref{perturbedmaximizerprob}):

\begin{equation}\label{discrete_argmax_ranges}
    \frac{\partial}{\partial \theta}f(\theta) =
        \begin{cases}
        (1,0) &\quad\text{if } \theta_1 > \theta_2+2\\
        (\frac{3}{4},\frac{1}{4}) &\quad\text{if }  \theta_2+2 >  \theta_1 > \theta_2\\
        (\frac{1}{4}, \frac{3}{4}) &\quad\text{if }\theta_2-2 < \theta_1 < \theta_2\\
        (0,1)  &\quad\text{if } \theta_1 < \theta_2-2
        \end{cases}
\end{equation}

\begin{definition} Subgradient and subdifferentiable.
A vector $\lambda$ is said to be a subgradient of a convex function $f$ at a point $\theta$ if 
\begin{equation}
    f(z) \geq f(\theta) + \langle \lambda,  z-\theta \rangle \quad\forall z
\end{equation}
The set of all subgradients of $f$ at $\theta$ is called the subdifferential of $f$ at $\theta$ and is denoted by 
 $\partial f(\theta)$. 
If $\partial f(\theta)$ is nonempty, $f$ is said to be subdifferentiable at $\theta$.
\end{definition} 

\textbf{Claim:} $\lambda = (\frac{1}{2},\frac{1}{2})$ is a subgradient of $f(\theta)$ at $\theta = (0,0)$. Note that $f((0,0)) =\frac{1}{2} $.
The proof requires showing that  
\begin{eqnarray}
        f(z) &\geq& f((0,0)) + \langle (\frac{1}{2},\frac{1}{2}),  z-(0,0) \rangle \quad\forall z \\ 
        f(z) &\geq& \frac{1}{2} + \langle (\frac{1}{2},\frac{1}{2}),  z \rangle \quad\forall z \\ 
        f(z) &\geq& \frac{1}{2} + \frac{1}{2}z_1 + \frac{1}{2}z_2 \quad\forall z \\ 
        2f(z) &\geq& 1 + z_1+ z_2 \quad\forall z,  \label{subgradienthalfhalf}
\end{eqnarray}
\begin{enumerate}
    \item In the case $z_1  \geq  z_2 +2$: 
    per Equation \ref{discrete_max_ranges}, $f(z) = z_1$, and the inequality $2z_1 \geq 1+z_1+z_2$  holds since $z_1 \geq 1+z_2$.
    \item In the case $z_2+2 \geq  z_1 \geq  z_2$, $f(z) = \frac{3}{4}\theta_1  + \frac{1}{4}\theta_2+ \frac{1}{2}$, and the inequality 
    \begin{eqnarray}
        1.5z_1+0.5z_2+1 &\geq& 1 + z_1+ z_2 \quad\forall z \\
        0.5z_1 &\geq& 0.5z_2 \quad\forall z 
    \end{eqnarray} holds in this case.
    \item The two other cases hold as they mirror these conditions.
\end{enumerate}

Which proves that $(\frac{1}{2},\frac{1}{2})$ is a subgradient of $f(\theta)$ at $\theta = (0,0)$.

\textbf{Claim:} $\lambda = (0.6,0.4)$ is a also subgradient of $f(\theta)$ at $\theta = (0,0)$.
The proof requires showing that  
\begin{eqnarray}
        f(z) &\geq& f((0,0)) + \langle (0.6,0.4),  z-(0,0) \rangle \quad\forall z \\ 
        f(z) &\geq& \frac{1}{2} + 0.6z_1 + 0.4z_2 \quad\forall z \label{subgradient.6}
\end{eqnarray}

\begin{enumerate}
    \item Consider the case $z_1 \geq z_2 +2$ , per Equation \ref{discrete_max_ranges}, $f(z) = z_1$, and the inequality $z_1 \geq \frac{1}{2}+0.6z_1+0.4z_2$  holds since
    \begin{eqnarray}
        z_1 &\geq& \frac{1}{2}+0.6z_1+0.4z_2\\
        0.4z_1 &\geq& \frac{1}{2}+0.4z_2\\
        z_1 &\geq& \frac{5}{4}+z_2.
    \end{eqnarray}
    \item In the case $z_2+2 \geq z_1 \geq z_2$, $f(z) = \frac{3}{4}z_1  + \frac{1}{4}z_2+ \frac{1}{2}$, and the inequality holds since 
\begin{eqnarray}
    \frac{3}{4}z_1  + \frac{1}{4}z_2+ \frac{1}{2} &\geq& \frac{1}{2}+0.6z_1+0.4z_2\\
    z_1 &\geq& z_2 .
\end{eqnarray}
        \item  The two other cases hold as they mirror these conditions.
\end{enumerate}

\textbf{Claim:} $\lambda = (0.8,0.2)$ is a  subgradient of $f(\theta)$ at $\theta = (2,0)$.
Note that $f((2,0)) = 2$. The proof requires showing that  
\begin{eqnarray}
        f(z) &\geq& f((2,0)) + \langle (0.8,0.2),  z-(2,0) \rangle \quad\forall z \\
        f(z) &\geq& 2 + 0.8z_1+0.2z_2- 1.6  \quad\forall z \\
        f(z) &\geq& 0.4 + 0.8z_1+0.2z_2  \quad\forall z 
\end{eqnarray}
\begin{enumerate}
    \item In the case $z_1 \geq  z_2 +2$ per Equation \ref{discrete_max_ranges}, $f(z) = z_1$, and the inequality holds
    \begin{eqnarray}
            z_1 &\geq& 0.4 + 0.8z_1+0.2z_2  \quad\forall z  \\
            0.2z_1 &\geq& 0.4 + 0.2z_2  \quad\forall z \\
            z_1 &\geq& 2 + z_2  \quad\forall z.
    \end{eqnarray}
    \item  In the case $z_2+2 \geq  z_1 \geq z_2$, $f(z) = \frac{3}{4}z_1  + \frac{1}{4}z_2+ \frac{1}{2}$, and the inequality holds since 
    \begin{eqnarray}
        \frac{3}{4}z_1  + \frac{1}{4}z_2+ \frac{1}{2} &\geq& 0.4+0.8z_1+0.2z_2\\
        2/40z_2+4/40 &\geq& 2/40z_1 \\
        z_2 +2 &\geq& z_1 
    \end{eqnarray}
    \item The two other cases hold as they mirror these conditions.
\end{enumerate}

\begin{figure}[ht]
\centering
\begin{subfigure}{.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/discrete_ranges_plot.jpg}
\end{subfigure}
\caption{Derivatives of $f(\theta)$.}
\label{fig:discrete_max_plot}
\end{figure}
\subsubsection{Generalizing the subgradient }
Just as $\lambda = (0.6,0.4)$ and $\lambda = (0.5,0.5)$ are subgradients of $f(\theta)$ at $\theta = (0,0)$, we next generalize the proof such that all $\lambda \in ((1/4,3/4),(3/4,1/4))$ are subgradients of $f(\theta)$ at $\theta = (0,0)$. The same proof can be used to show that all $\lambda \in ((3/4,1/4),(1,0))$ are subgradients of $f(\theta)$ at $\theta = (2,0)$, and similarly,  all $\lambda \in ((0,1),(1/4,3/4))$ are subgradients of $f(\theta)$ at $\theta = (0,2)$.

\begin{definition} Directional derivative. 
Let $f$ be any function from $\R^n$ to $[-\infty, \infty]$ ,  and let $\theta$ be a point where $f$ is finite.
The one-sided directional derivative of $f$ at $\theta$ with respect to a vector $\delta$ is defined to be the limit
\begin{equation}
    f'(\theta;\delta) = lim_{\epsilon \downarrow 0} \frac{f(\theta+\epsilon \delta) - f(\theta)}{\epsilon}
\end{equation}
if it exists.
\end{definition} 

\paragraph{Rockafellar's Theorem 23.2, \cite{rockafellar-1970a}}
Let $f$ be a convex function, and let $\theta$ be a point in which $f$ is finite. Then $\lambda$ is a subgradient of $f$ at point $\theta$ if and only if
\begin{equation}
    f'(\theta;\delta) \geq \langle \lambda,\delta \rangle, \;   \forall \delta.
\end{equation}

\begin{theorem}
For the expected perturbed maximum for discrete random variable perturbations $f(\theta)$ as defined in this section, the range of the probabilities of the perturbed maximizer (maximizing argument) (Equation \ref{perturbedmaximizerprob}) is the probability simplex $\Delta = \{(x_1,x_2): \sum_{i=1}^2 x_i =1 , \: x_i \geq 0  \: \forall i \in \{1,2\} \}
$.
\end{theorem}
\begin{proof}
     The derivative of the expected perturbed maximum  $f(\theta)$, $\frac{\partial}{\partial \theta}f(\theta) = (\frac{\partial}{\partial \theta_1}f(\theta), \frac{\partial}{\partial \theta_2}f(\theta))$ corresponds to the probabilities of the maximizer $(P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 1 \right),P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 2 \right))$  (Equation \ref{perturbedmaximizerprob}). 
     \textcolor{blue}{It holds that the range of subgradients of $f(\theta)$ on its domain is equal to the probability simplex, $ \text{range }  \partial f = \Delta $}.
    Specifically, Corollary \ref{subgradients_at_zerozero} proves that the maximizer probabilities $\lambda \in [(1/4,3/4),(3/4,1/4)]$ are subgradients of $f(\theta)$ at $\theta = (0,0)$.
    The proof technique of Corollary \ref{subgradients_at_zerozero} can be used to show that all $\lambda \in ((3/4,1/4),(1,0))$ are subgradients of $f(\theta)$ at $\theta = (2,0)$, and similarly,  all $\lambda \in ((0,1),(1/4,3/4))$ are subgradients of $f(\theta)$ at $\theta = (0,2)$.
\end{proof}
\begin{corollary}\label{subgradients_at_zerozero}
For $f(\theta)$ as defined in this section (Section \ref{expectedmax_discretechapter}), all $\lambda \in [(1/4,3/4),(3/4,1/4)]$, i.e., $\lambda_2 = 1- \lambda_1$ , $\frac{3}{4}  \geq \lambda_1\geq \frac{1}{4}$, are subgradients of $f(\theta)$ at $\theta = (0,0)$.
\end{corollary}
\begin{proof}
    $f(\theta)$ is convex (Corollary \ref{convexity}) and proper, therefore Rockafellar's Theorem 23.2 can be applied.
    The proof follows by showing that for said subgradient range, it holds per Theorem 23.2 \cite{rockafellar-1970a} that
\begin{equation}\label{theoren232_zerozero}
    f'((0,0);\delta) \geq \langle \lambda,\delta \rangle, \;   \forall \delta.
\end{equation}

First, $f'((0,0);\delta)$ evaluates to
\begin{eqnarray}\label{lim_at_zerozero}
    f'((0,0);\delta) &=& lim_{\epsilon \downarrow 0} \frac{f((0,0)+\epsilon \delta) - f((0,0)}{\epsilon} \\
     &=& lim_{\epsilon \downarrow 0} \frac{f(\epsilon \delta) - f((0,0)}{\epsilon} \\
     &=& lim_{\epsilon \downarrow 0} \frac{f(\epsilon\delta_1,\epsilon\delta_2) - \frac{1}{2}}{\epsilon} 
\end{eqnarray}

Consider first $\delta= (\delta_2,\delta_1) \in [(-1,-1),(1,1)]: \delta_2 \leq \delta_1$, as illustrated in Figure \ref{fig:dd_delta1half}.
\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\includegraphics[width=\linewidth]{figures/dd_delta1half.jpg}
\end{subfigure}
\caption{Illustration of $\delta= (\delta_2,\delta_1) \in [(-1,-1),(1,1)]: \delta_2 \leq \delta_1$ for $\theta_1 = \theta_2$. }
\label{fig:dd_delta1half}
\end{figure}

In this range, $\delta_2+2 \geq \delta_1 \geq \delta_2$, and $f(\delta)= \frac{3}{4}\delta_1  + \frac{1}{4}\delta_2+ \frac{1}{2}$.
Equation \ref{lim_at_zerozero} evaluates to 
\begin{eqnarray}\label{lim_at_zerozero_1}
    f'((0,0);\delta) &=& lim_{\epsilon \downarrow 0} \frac{\frac{3}{4}\epsilon \delta_1 + \frac{1}{4}\epsilon \delta_2+ \frac{1}{2} - \frac{1}{2}}{\epsilon} \\
    &=& \frac{3}{4}\delta_1 + \frac{1}{4}\delta_2.
\end{eqnarray}
Therefore Equation \ref{theoren232_zerozero} for mentioned $\delta= (\delta_2,\delta_1) \in [(-1,-1),(1,1)]: \delta_1 \leq \delta_2$ holds since
\begin{eqnarray}
    \frac{3}{4}\delta_1 + \frac{1}{4}\delta_2  &\geq& \lambda_1\delta_1 +\lambda_2\delta_2, \;   \forall \delta_1 \leq \delta_2 \\
     &\geq& \lambda_1\delta_1 +(1-\lambda_1)\delta_2, \;   \forall \delta_2 \leq \delta_1 \\
     &\geq& (\frac{3}{4} -\epsilon)\delta_1 + (\frac{1}{4} +\epsilon)\delta_2, \;   \forall \frac{1}{2} \geq \epsilon \geq 0 \;   ,  \delta_2 \leq \delta_1 \\
     &\geq& \frac{3}{4}\delta_1+ \frac{1}{4} \delta_2 -\epsilon(\delta_1-\delta_2), \;   \forall \frac{1}{2} \geq \epsilon \geq 0 \;   ,  \delta_2 \leq \delta_1 
\end{eqnarray}
when we set $\lambda_2 = 1- \lambda_1$, for $\frac{3}{4}  \geq \lambda_1\geq \frac{1}{4}$. The last equality holds since $\delta_2 \leq \delta_1 $.

The same technique can be applied to the complementary range $\delta= (\delta_2,\delta_1) \in [(1,1),(-1,-1)]: \delta_1 \leq \delta_2$.
In this range, $\delta_2+2 \leq \delta_1 \leq \delta_2$, and $f(\delta)= \frac{3}{4}\delta_2  + \frac{1}{4}\delta_1+ \frac{1}{2}$.
Equation \ref{lim_at_zerozero} then evaluates to 
\begin{eqnarray}\label{lim_at_zerozero_2}
    f'((0,0);\delta) &=& lim_{\epsilon \downarrow 0} \frac{\frac{3}{4}\epsilon \delta_2+ \frac{1}{4}\epsilon \delta_1+ \frac{1}{2} - \frac{1}{2}}{\epsilon} \\
    &=& \frac{3}{4}\delta_2 + \frac{1}{4}\delta_1 .
\end{eqnarray}
Therefore, Equation \ref{theoren232_zerozero} for mentioned $\delta= (\delta_2,\delta_1) \in [(-1,-1),(1,1)]: \delta_1 \leq \delta_2$ holds since
\begin{eqnarray}
    \frac{3}{4}\delta_2 + \frac{1}{4}\delta_1 &\geq& \lambda_2\delta_2 +\lambda_1\delta_1 , \;\forall \delta_1 \leq \delta_2\\
     &\geq& \lambda_2\delta_2 +(1-\lambda_2)\delta_1, \;   \forall \delta_1 \leq \delta_2 \\
     &\geq& (\frac{3}{4} -\epsilon)\delta_2 + (\frac{1}{4} +\epsilon)\delta_1, \;   \forall \frac{1}{2} \geq \epsilon \geq 0 \;   ,  \delta_1 \leq \delta_2 \\
     &\geq& \frac{3}{4}\delta_2+ \frac{1}{4} \delta_1 -\epsilon(\delta_2-\delta_1), \;   \forall \frac{1}{2} \geq \epsilon \geq 0 \;   ,  \delta_1 \leq \delta_2 .
\end{eqnarray}
\iffalse when we set $\lambda_1 = 1- \lambda_2$, for $\frac{3}{4}  \geq \lambda_2\geq \frac{1}{4}$. The last equality holds since $\delta_1 \leq \delta_2 $.
\fi




\end{proof}
To conclude this analysis, the range of derivatives of the perturbed expected max with discrete random variables is the probability simplex.

\subsection{The expected perturbed maximum for smooth bounded random variable perturbations}\label{expectedmax_smoothbounded}

For $\theta \in \R^2$, and for i.i.d. random variables with a smooth bounded probability density function $\gamma \sim U(1,-1)$. Let 
\begin{equation}\label{f_theta_boundedsmooth_definition}
    f(\theta) = \E_{\gamma \sim U(1,-1)} \left[ \max_{i}\{ \theta_i+ \gamma_i\} \right]
\end{equation}
denote the expected perturbed maximum over the domain $\mathcal{C} =\R^d$. Let $f(\theta)$ take values over the extended real domain $\R \cup \{\pm \infty\}$. Clearly, $P(1= \arg \max_i \{\theta_i+\gamma_i \}) = P(\theta_1+\gamma_1 \geq \theta_2+\gamma_2)$.

\begin{eqnarray}
    f(\theta) &=& \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max_i\{ \theta_i+ \gamma_i\} \right] \\
    &=& \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max\{ \theta_1+ \gamma_1 ,\theta_2+ \gamma_2  \} \right]  - E_{\gamma_2 \sim [-1,1]} \left[ \gamma_2 \right]\\
    &=& \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max\{ \theta_1+ \gamma_1 ,\theta_2+ \gamma_2  \}  - \gamma_2 \right] \\
    &=& \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max\{ \theta_1+ \gamma_1 -\gamma_2 ,\theta_2 \}  +\theta_2-\theta_2 \right] \\
    &=&\theta_2 + \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max\{ \theta_1-\theta_2 + \gamma_1 -\gamma_2 ,0 \}  \right]
\end{eqnarray}

The second equation holds since $E_{\gamma_2 \sim [-1,1]} \left[ \gamma_2 \right] =0$. 

Define $\theta = \theta_1-\theta_2$ and $Z = \gamma_1-\gamma_2$. Then, the random variable $Z$ has a triangular distribution. The random variable $Z$ has the following CDF (Figure \ref{fig:smoothuniformcdf}):
\begin{eqnarray}
    F_{Z}(z) &=& P(\gamma_1-\gamma_2 \leq z) \\
    &=& 
    \begin{cases}
        0 \quad\text{if }  z < -2 \\ 
        \frac{1}{4}\frac{(2+z)^2}{2} \quad\text{if } 0 > z \geq -2\\
         \frac{1}{4}(4-\frac{(2-z)^2}{2}) \quad\text{if } 2 \geq z \geq 0 \\ 
        0 \quad\text{if }  z > 2 
    \end{cases}
\end{eqnarray}
\iffalse An alternative approach:  \href{https://easysas.blogspot.com/2013/04/distribution-of-difference-of-two.html} \fi 
\begin{figure}[ht!]
\centering
\begin{subfigure}{.7\textwidth}
\centering\includegraphics[width=\linewidth]{figures/smoothuniformcdf.jpg}
\end{subfigure}
\caption{Illustration of the CDF and PDF of the random variable $Z= \gamma_1-\gamma_2 ,  \gamma_1,\gamma_2 \sim U(-1,1)$.}
\label{fig:smoothuniformcdf}
\end{figure}

\begin{figure}[h]
\centering
\begin{subfigure}{.3\textwidth}
\centering\includegraphics[width=\linewidth]{figures/simulated_pdf_z.png}
\end{subfigure}
\caption{Simulation of the density of the difference between 1M iid uniform(-1,1) random variables.}
\label{fig:simulated_pdf_z}
\end{figure}


The random variable $Z$ has the following pdf, also verified in simulation of the density of the difference between 1M iid Uniform(-1,1) random variables (Figure \ref{fig:simulated_pdf_z}):
\begin{eqnarray}\label{pdf_smoothbounded}
    f_{Z}(z) &=& 
    \begin{cases}
        \frac{1}{4}(2+z) \quad\text{if } 0 > z \geq -2\\
        \frac{1}{4}(2-z) \quad\text{if } 2 \geq z \geq 0 \\ 
         0 \quad\text{otherwise } 
    \end{cases}
\end{eqnarray}

With the pdf of the random variable $Z$ (Equation \ref{pdf_smoothbounded}) consider $f(\theta)$ the appropriate range of $\theta$.

\begin{enumerate}
\item \textbf{Case: $-\theta < -2$} 

In this case $\theta_1-\theta_2 > 2$, therefore
\begin{align}
    f(\theta) &= \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max_i\{ \theta_i+ \gamma_i\} \right] \\
    &= \E_{\gamma_1 \sim [-1,1]} \left[ \theta_1+ \gamma_1\ \right] \\ 
    &= \theta_1+ \E_{\gamma_1 \sim [-1,1]} \left[\gamma_1\ \right] \\
    &= \theta_1
\end{align}

\item \textbf{Case: $0 \leq -\theta \leq 2$} 
 (Figure \ref{fig:smoothuniformpdf_case1})
\begin{figure}[h!]
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/integral_max_bounded.jpg}
\end{subfigure}
\caption{Illustration of the integral area of the pdf of Z in the case that $0 \leq -\theta \leq 2$.}
\label{fig:smoothuniformpdf_case1}
\end{figure}
{\allowdisplaybreaks
\begin{align}
    f(\theta) &= \theta_2 + \E_{z} \left[ \max\{ \theta + z ,0 \}  \right] \\
    &= \theta_2 + \int_{-\theta}^{2} f_Z(z)( \theta + z) dz \label{eq:f_smoothbounded1}\\
    &= \theta_2 + \int_{-\theta}^{2} \frac{1}{4}(2-z)( \theta + z) dz \\
    &= \theta_2 + \int_{-\theta}^{2} \frac{1}{4}(2\theta +2z - z\theta -z^2) dz \\
    &= \theta_2 + \frac{1}{2} \int_{-\theta}^{2} \theta dz + \frac{1}{2} \int_{-\theta}^{2}  z dz - \frac{1}{4}\int_{-\theta}^{2} z \theta dz - \frac{1}{4}\int_{-\theta}^{2}  z^2 dz  \\
    &= \theta_2 +  \frac{1}{2}\left[  \theta z \right]_{-\theta}^2 + \frac{1}{2} \left[  \frac{z^2}{2} \right]_{-\theta}^2 - \frac{1}{4} \left[  \frac{z^2\theta}{2} \right]_{-\theta}^2 - \frac{1}{4} \left[  \frac{z^3}{3} \right]_{-\theta}^2 \\
    &= \theta_2 + \frac{1}{2}(2+\theta)\theta +1- \frac{\theta^2}{4} -(\frac{1}{2}\theta- \frac{\theta^3}{8}) - (\frac{2}{3}+\frac{\theta^3}{12})\\
    &= \theta_2 + \frac{1}{3} + \frac{1}{2}\theta +\frac{1}{4}\theta^2 + \frac{1}{24}\theta^3 \\
    &= \theta_2 +  \frac{1}{4} \left(\frac{4}{3} +2\theta + \theta^2 +\frac{\theta^3}{6} \right)\\
    &= \theta_2 +  \frac{1}{4} \left(\frac{4}{3} +2(\theta_1-\theta_2) + (\theta_1-\theta_2)^2 +\frac{(\theta_1-\theta_2)^3}{6} \right)\\
    &= \theta_2 +  \frac{1}{4} \left(\frac{4}{3} +2\theta_1-2\theta_2+ \theta_1^2+\theta_2^2-2 \theta_1 \theta_2 + \frac{\theta_1^3 - 3 \theta_1^2 \theta_2+ 3 \theta_1 \theta_2^2 - \theta_2^3}{6} \right) \\
    &= \frac{1}{4} \left(\frac{4}{3} +2\theta_1 + 2\theta_2+ \theta_1^2+\theta_2^2-2 \theta_1 \theta_2 + \frac{\theta_1^3 - 3 \theta_1^2 \theta_2+ 3 \theta_1 \theta_2^2 - \theta_2^3}{6} \right) \\
     &= \frac{1}{4} \left(\frac{4}{3} +2(\theta_1 + \theta_2)+ (\theta_1-\theta_2)^2 + \frac{1}{6}(\theta_1-\theta_2)^3\right)
\end{align}
}


\item \textbf{Case: $-2 \leq -\theta \leq 0$}  
{\allowdisplaybreaks
\begin{align}
    f(\theta) &= \theta_2 + \E_{z} \left[ \max\{ \theta + z ,0 \}  \right] \\
    &= \theta_2 + \int_{-\theta}^{0} f_Z(z)( \theta + z) dz + \int_{0}^{2} f_Z(z)( \theta + z) dz \\
    &= \theta_2 + \int_{-\theta}^{0} \frac{1}{4}(2+ z)(\theta +z) dz + \int_{0}^{2} \frac{1}{4}(2- z)(\theta +z) dz  \\
     &= \theta_2 + \frac{1}{4}(\theta^2- \frac{1}{6} \theta^3) + \frac{1}{4}(2 \theta +\frac{4}{3} ) \\
     &= \theta_2 + \frac{1}{4}(\theta^2- \frac{1}{6} \theta^3 + 2 \theta +\frac{4}{3} )\\
     &= \frac{1}{4} \left(\frac{4}{3}+ 2 (\theta_1+\theta_2) +(\theta_1-\theta_2)^2 -\frac{1}{6}(\theta_1-\theta_2)^3 \right)
\end{align}

\begin{align}
   \int_{-\theta}^{0}  \frac{1}{4}(2+ z)(\theta +z)dz  &= \frac{1}{2} \int_{-\theta}^{0} \theta dz + \frac{1}{2} \int_{-\theta}^{0}  z dz + \frac{1}{4}\int_{-\theta}^{0} z \theta dz + \frac{1}{4}\int_{-\theta}^{0} z^2 dz   \\
    &= \frac{1}{2}\left[  \theta z \right]_{-\theta}^0 + \frac{1}{2} \left[  \frac{z^2}{2} \right]_{-\theta}^0 + \frac{1}{4} \left[  \frac{z^2\theta}{2} \right]_{-\theta}^0 + \frac{1}{4} \left[  \frac{z^3}{3} \right]_{-\theta}^0 \\ 
    &= \frac{1}{2} \theta^2 - \frac{1}{4}\theta^2 -\frac{1}{8} \theta^3 +\frac{1}{12}\theta^3 \\
    &= \frac{1}{4}(\theta^2- \frac{1}{6} \theta^3)
\end{align}

\begin{align}
    \int_{0}^{2} \frac{1}{4}(2-z)( \theta + z) dz
    &=  \int_{0}^{2}  \frac{1}{4}(2\theta +2z - z\theta -z^2) dz \\
    &=  \frac{1}{2} \int_{0}^{2} \theta dz + \frac{1}{2} \int_{0}^{2} z dz - \frac{1}{4}\int_{0}^{2} z \theta dz - \frac{1}{4}\int_{0}^{2}  z^2 dz  \\
    &=  \frac{1}{2}\left[  \theta z \right]_0^2 + \frac{1}{2} \left[  \frac{z^2}{2} \right]_0^2 - \frac{1}{4} \left[  \frac{z^2\theta}{2} \right]_0^2- \frac{1}{4} \left[  \frac{z^3}{3} \right]_0^2 \\
    &=  \theta +1 - \frac{1}{2} \theta -\frac{2}{3} \\
    &= \frac{1}{2} \theta +\frac{1}{3} \\
    &= \frac{1}{4}(2 \theta +\frac{4}{3} )
\end{align}
    
\item \textbf{Case: $-\theta > 2$} 

In this case $\theta_1-\theta_2 < -2$,  therefore
\begin{align}
    f(\theta) &= \E_{\gamma_1,\gamma_2 \sim [-1,1]} \left[ \max_i\{ \theta_i+ \gamma_i\} \right] \\
    &= \E_{\gamma_2 \sim [-1,1]} \left[ \theta_2+ \gamma_2\ \right] \\ 
    &= \theta_2+ \E_{\gamma_2 \sim [-1,1]} \left[\gamma_2\ \right] \\
    &= \theta_2
\end{align}
}
\end{enumerate}

To conclude, 
\begin{align}\label{ftheta_boundedsmooth}
    f(\theta) &=
    \begin{cases}
        \theta_1 \quad\text{if }  -\theta < -2 \\ 
        \frac{1}{4} \left(\frac{4}{3} +2(\theta_1 + \theta_2)+ (\theta_1-\theta_2)^2 + \frac{1}{6}(\theta_1-\theta_2)^3\right)    \quad\text{if } 0 \leq -\theta \leq 2 \\
        \frac{1}{4} \left(\frac{4}{3}+ 2 (\theta_1+\theta_2) +(\theta_1-\theta_2)^2 -\frac{1}{6}(\theta_1-\theta_2)^3 \right) \quad\text{if } -2 \leq -\theta \leq 0 \\ 
        \theta_2 \quad\text{if }  -\theta > 2
    \end{cases}
\end{align}

Alternatively, one writes 
\begin{align}\label{ftheta_boundedsmooth_}
    f(\theta) &=
    \begin{cases}
        \theta_1 \quad\text{if }  \theta > 2 \\ 
        \frac{1}{4} \left(\frac{4}{3}+ 2 (\theta_1+\theta_2) +(\theta_1-\theta_2)^2 -\frac{1}{6}(\theta_1-\theta_2)^3 \right) \quad\text{if } 2 \geq \theta \geq 0 \\ 
        \frac{1}{4} \left(\frac{4}{3} +2(\theta_1 + \theta_2)+ (\theta_1-\theta_2)^2 + \frac{1}{6}(\theta_1-\theta_2)^3\right)  \quad\text{if } 0 \geq \theta \geq -2 \\
        \theta_2 \quad\text{if }  \theta < -2
    \end{cases}
\end{align}
$f(\theta)$ for $\theta_2=0$ is illustrated in Figure \ref{fig:ftheta_boundedsmooth_theta_ranges_plot}.


\begin{figure}[ht!]
\centering
\begin{subfigure}{.55\textwidth}
  \centering\includegraphics[width=\linewidth]{figures/ftheta_boundedsmooth_theta_ranges_plot.jpg}
\end{subfigure}
\caption{Illustration of $f(\theta)$ for $\theta_2=0$.}
\label{fig:ftheta_boundedsmooth_theta_ranges_plot}
\end{figure}

%To Do -Prove smoothness  of $f(\theta)$ (Equation \ref{ftheta_boundedsmooth}).

\subsubsection{The derivative of the perturbed expected max }
The derivative of $f(\theta)$ (Equation \ref{ftheta_boundedsmooth}), $\frac{\partial}{\partial \theta}f(\theta) = (\frac{\partial}{\partial \theta_1}f(\theta), \frac{\partial}{\partial \theta_2}f(\theta))$ corresponds to the probabilities of the arg max, $(P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 1 \right),P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 2 \right))$  (Equation \ref{perturbedmaximizerprob})


\begin{align}\label{maximizer_prob_boundedsmooth}
    \frac{\partial}{\partial \theta}f(\theta) &=
    \begin{cases}
        (1,0) \quad\text{if }  -\theta < -2 \\ 
        (\frac{1}{2}+ \frac{1}{2}\theta+ \frac{1}{8}\theta^2, \frac{1}{2}- \frac{1}{2}\theta - \frac{1}{8}\theta^2) \quad\text{if } 0 \leq -\theta \leq 2 \\
       (\frac{1}{2}+\frac{1}{2}\theta-\frac{1}{8}\theta^2,\frac{1}{2}-\frac{1}{2}\theta + \frac{1}{8}\theta^2 ) \quad\text{if } -2 \leq -\theta \leq 0 \\ 
       (0,1)\quad\text{if }  -\theta > 2
    \end{cases}
\end{align}

\begin{align}
    \frac{\partial}{\partial \theta}f(\theta) &=
    \begin{cases}
        (1,0) \quad\text{if }  \theta > 2 \\ 
        (\frac{1}{2}+\frac{1}{2}\theta-\frac{1}{8}\theta^2,\frac{1}{2}-\frac{1}{2}\theta + \frac{1}{8}\theta^2 ) \quad\text{if } 2 \geq \theta \geq 0 \\ 
        (\frac{1}{2}+ \frac{1}{2}\theta+ \frac{1}{8}\theta^2, \frac{1}{2}- \frac{1}{2}\theta - \frac{1}{8}\theta^2) \quad\text{if } 0 \geq \theta \geq -2 \\
       (0,1)\quad\text{if }  \theta < -2
    \end{cases}
\end{align}

$\frac{\partial}{\partial \theta}f(\theta)$ is illustrated in Figure \ref{fig:ftheta_derivatives_boundedsmooth_theta_ranges_plot}.

\begin{figure}[ht!]
\centering
\begin{subfigure}{.55\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/ftheta_derivatives_boundedsmooth_theta_ranges_plot.jpg}
\end{subfigure}
\caption{Illustration of $\frac{\partial}{\partial \theta_1}f(\theta)$ and $\frac{\partial}{\partial \theta_2}f(\theta)$, corresponding to $P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 1 \right)$ and $P_\gamma \left(\arg \max _i \{ \theta_i+ \gamma_i \} = 2 \right)$ respectively.}
\label{fig:ftheta_derivatives_boundedsmooth_theta_ranges_plot}
\end{figure}



Then, the partial derivatives $\frac{\partial}{\partial \theta}f(\theta) \in [0,1]$ and sum to $1$, as expected.
\begin{equation}
    \frac{\partial}{\partial \theta_1}f(\theta)+ \frac{\partial}{\partial \theta_2}f(\theta) = 1
\end{equation} 

\begin{enumerate}
\item \textbf{Case: $0 \leq -\theta \leq 2$} 
\begin{align}
    \frac{\partial}{\partial \theta}f(\theta) &=(\frac{1}{4}(2 + 2\theta_1-2\theta_2 +\frac{3\theta_1^2-6\theta_1\theta_2+3\theta_2^2}{6}), \frac{1}{4}(2 + 2\theta_2-2\theta_1 + \frac{-3\theta_1^2+6\theta_1\theta_2-3\theta_2^2}{6})) \\ 
    &= (\frac{1}{2}+ \frac{1}{2}(\theta_1-\theta_2)+ \frac{1}{8}(\theta_1-\theta_2)^2, \frac{1}{2}- \frac{1}{2}(\theta_1-\theta_2) - \frac{1}{8}(\theta_1-\theta_2)^2) \\
    &=(\frac{1}{2}+ \frac{1}{2}\theta+ \frac{1}{8}\theta^2, \frac{1}{2}- \frac{1}{2}\theta - \frac{1}{8}\theta^2)
\end{align}

The global minimum of the derivative $f(\theta)$ w.r.t. $\theta_1$,  $ \min \frac{\partial}{\partial \theta_1}f(\theta) = 0$ for $\theta = -2$, since
\begin{equation}
    \frac{\partial \frac{1}{4}(2 + 2\theta_1-2\theta_2 +\frac{3\theta_1^2-6\theta_1\theta_2+3\theta_2^2}{6})}{\partial \theta_1}= 
    \frac{1}{4}(2 +\theta_1 -\theta_2),
\end{equation}
in which case $\frac{\partial}{\partial \theta_2}f(\theta) = 1$.
The global maximum of the derivative $f(\theta)$ w.r.t. $\theta_1$,  $ \max \frac{\partial}{\partial \theta_1}f(\theta) = \frac{1}{2}$ for $-\theta = 0$, in which case $\frac{\partial}{\partial \theta_2}f(\theta) = \frac{1}{2}$.

The global maximum of the derivative $f(\theta)$ w.r.t. $\theta_2$,  $ \max \frac{\partial}{\partial \theta_2}f(\theta) = 1$ for $\theta_2 = \theta_1+2$, since
\begin{equation}
    \frac{\partial \frac{1}{4}(2 + 2\theta_2-2\theta_1 + \frac{-3\theta_1^2+6\theta_1\theta_2-3\theta_2^2}{6}))}{\partial \theta_2}= 
    \frac{1}{4}(2 +\theta_1 -\theta_2),
\end{equation}
in which case $\frac{\partial}{\partial \theta_1}f(\theta) = 0$.
The global minimum of the derivative $f(\theta)$ w.r.t. $\theta_2$,  $ \max \frac{\partial}{\partial \theta_2}f(\theta) = \frac{1}{2}$ for $-\theta = 0$, in which case $\frac{\partial}{\partial \theta_1}f(\theta) = \frac{1}{2}$.
\end{enumerate}

\begin{theorem}
The range of the probabilities of the perturbed maximizer (maximizing argument) (Equation \ref{perturbedmaximizerprob}), of the expected perturbed maximum function as defined in Equation \ref{f_theta_boundedsmooth_definition}, equals the probability simplex, denoted $\Delta$, such that 
\begin{equation}
    \cup \{ P_\gamma \left(\arg \max _{i} \{ \theta_i+ \gamma_i \} = j  \right) \} = \Delta.
\end{equation}
\end{theorem}

\begin{proof}    
Recall that the derivative of the expected perturbed maximum  $f(\theta)$ is the probability of the expected maximizer (Equation \ref{perturbedmaximizerprob}).  $f(\theta)$ (Equation \ref{f_theta_boundedsmooth_definition}) is a closed proper convex function on $R^d$ (Theorem \ref{PerturbedMaximizers}), then per Corollary 23.5.1 and (beginning of chapter 24) \cite{rockafellar-1970a} the following holds for 
the range of $\partial f $:
\begin{equation}
   ri( dom f^*) \subset \text{range } \partial f \subset dom f^*,
\end{equation}
    where 
    \begin{equation}
        \text{range }  \partial f  = \cup \{ \partial f(\theta) | \theta \in R^n \}.
    \end{equation}

It holds that $domf^* \subseteq \Delta$, since 
$domf^* \subseteq \{\lambda \in \R^d: \sum_{y} \lambda_y=1, \lambda_y \geq 0 \;  \forall \lambda_y\}$ (Equations \ref{expectedmaximizer_probabilities}, and \ref{conjugate_cases_max}).
The function $f(\theta)$ takes values over the extended real domain $\R \cup \{\pm \infty\}$ and its domain is in a subset of $\R^d$. 
Then, $dom f^* $ is a convex set in $\R^d$ \iffalse, since it is the image of the convex set of the epigraph of $f$ under linear transformation \fi (Theorem 3.4, \cite{rockafellar-1970a}).
The probability simplex's extreme points are members of  $\text{range } \partial f$ (Equation \ref{maximizer_prob_boundedsmooth}), and $\text{range } \partial f \subset dom f^*$ (Equation  \ref{rockafellar_rangedf}, \cite{rockafellar-1970a}). Then, since $dom f^*$ is a convex set, $dom f^*$ must be the convex hull of these extreme points, which is the probability simplex $\Delta$. 
Since $ ri( dom f^*) \subset \text{range } \partial f$ (Equation  \ref{rockafellar_rangedf}, \cite{rockafellar-1970a}), and we concluded that $ri(\Delta) = ri( dom f^*)$, it must be that $\text{range } \partial f = \Delta$.
\end{proof}


\subsection{Summary}
The difference between the properties of the probabilities models is that for a smooth unbounded probability the expected perturbed maximum $f(\theta)$ is essentially smooth, therefore the probability is a single-valued mapping (Theorem \ref{theorem1}).
For discrete random  perturbations, this property is not guaranteed since $f(\theta)$ is not essentially smooth.



\begin{corollary}
Let $f(\theta) = \E_{\gamma \sim \mathcal{G}} \left[ \max_i\{ \theta_i+ \gamma_i\} \right]$, $\theta, \gamma \in \R^d$  where $\gamma_i$ are i.i.d. random variables that follow a probability distribution $\mathcal{G}$ with a smooth probability density function.
Then, the representation of $f(\theta)$ is overcomplete when $f(\theta)$ is not strictly convex, and minimal otherwise. 
\end{corollary}

\begin{proof}
$f(\theta)$ is convex (Corollary \ref{convexity}). Therefore, for every $\lambda \in [0,1]$, and $\theta, \theta' \in \R^d$ it holds that 
\begin{equation}\label{f_max_convex}
    f(\lambda \theta+ (1-\lambda) \theta') \leq \lambda f(\theta)+ (1-\lambda)f( \theta')
\end{equation}

Explicitly,
\begin{equation}
    f(\lambda \theta+ (1-\lambda) \theta') =
    \E_{\gamma \sim \mathcal{G}} \left[ \max_i\{ \lambda(\theta_i+ \gamma_i) +(1-\lambda)(\theta'_i+ \gamma'_i) \} \right],
\end{equation}
and
\begin{eqnarray}
    \lambda f(\theta)+ (1-\lambda)f( \theta') &=& \lambda  \E_{\gamma \sim \mathcal{G}} \left[ \max_i\{\theta_i+ \gamma_i \} \right] + (1-\lambda)  \E_{\gamma \sim \mathcal{G}} \left[ \max_i\{ \theta'_i+ \gamma'_i \} \right] \\
    &=& \E_{\gamma \sim \mathcal{G}} \left[ \lambda \max_i\{ \theta_i+ \gamma_i \}+ (1-\lambda)\max_i\{ \theta'_i+ \gamma'_i \} \right] \\
    &=& \E_{\gamma \sim \mathcal{G}} \left[\max_i\{ \lambda (\theta_i+ \gamma_i) + \max_i\{ (1-\lambda) (\theta'_i+ \gamma'_i)  \right] 
\end{eqnarray}

Assume that the function $f(\theta)$ is not strictly convex. Meaning, there exist $\theta$ and $\theta'$ such that
\begin{equation}\label{f_max_convex}
    f(\lambda \theta+ (1-\lambda) \theta') = \lambda f(\theta)+ (1-\lambda)f( \theta')
\end{equation}

for any $\lambda \in [0,1]$ and $\gamma \sim \mathcal{G}$, suggesting that $f(\theta)$ is linear on the segment $[\theta+\gamma, \theta' + \gamma']$.

For $d=1$, indeed $f(\theta)$ is linear on the segment $[\theta+\gamma, \theta' + \gamma']$ as it is a linear combination of two scalars.
For $d>1$, however, $f(\theta)$ is piece-wise constant function, unless $\theta= \theta'$, which happens with probability zero.
\end{proof}



==> logsumexp.tex <==
\section{The expected perturbed log-sum-exp for random variable perturbations}\label{log-sum-exp}

For $\theta \in \R^d$ and i.i.d. random variables $\gamma \in \R^d$ perturbations (i.e., discrete or smooth), define 
\begin{equation}\label{f_theta_logsumexp_perturbed}
    f(\theta) = \E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right]
\end{equation} with domain $R^d$, and values over the extended real domain $f(\theta) : \R^d \rightarrow \R \cup \{\pm \infty\}$.

\begin{corollary}
    The range of the probabilities of the state variables of the expected perturbed log-sum-exp function as defined in Equation \ref{f_theta_logsumexp_perturbed}, differs very little from the probability simplex, $\Delta$, such that 
    \begin{equation}
        ri( \Delta) \subset \text{range }  p_\gamma  \subset \Delta,
    \end{equation}
\end{corollary}

\begin{proof}
The derivatives of the expected perturbed log-sum-exp  $f(\theta)$ (Equation \ref{f_theta_logsumexp_perturbed}) are a probability function. 
The derivative of $f(\theta)$ w.r.t. $\theta_j$ is
\begin{equation}\label{logsumexp_derivative}
    \frac{\partial f(\theta)}{\partial \theta_j} = \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right].
\end{equation}

The derivatives are probability a function. Denote $\frac{\partial f(\theta)}{\partial \theta_j}$ by $p_{\gamma,j}$ and note that $\sum_{j=1}^{d} p_{\gamma,j} =1, p_{\gamma,j} \geq 0  \quad \forall j$.
\begin{equation}\label{log_sum_exp_conjgate_prob}
    \sum_{j=1}^{d} p_{\gamma,j} = \sum_{j=1}^{d}\E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  = \E_\gamma \left[\sum_{j=1}^{d}\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d}  e^{\theta_i+\gamma_i}} \right] =1
\end{equation}

\begin{equation}\label{log_sum_exp_conjgate_prob_nonneg}
    \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right] \geq 0  \quad \forall j
\end{equation}

\textcolor{blue}{If we define $f(\theta) = \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i})$ then $\frac{\partial f(\theta)}{\partial \theta_j}$ is the probability of state $j$, since 
$\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}}= P_\gamma(\theta_j)$,  
a Gibbs model.}

Further, the convex conjugate of $f(\theta)$ is
\begin{equation}
    f^{*}\left(\lambda\right):=\sup _{\theta\in \R^d} \{\langle \theta,\lambda \rangle - \E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right] \}.
\end{equation}

Derivative w.r.t. $\theta_j$ and apply Leibniz's integral rule for differentiation under the integral sign, which can be applied since $\E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right]$ is a continuous and continuously differentiable function,
\begin{eqnarray}
    \frac{\partial}{\partial \theta_j} \left( \sum_{i=1}^{d} \theta_i \lambda_i - \E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right] \right) &=&
    \frac{\partial}{\partial \theta_j} \left( \sum_{i=1}^{d} \theta_i \lambda_i \right)- \frac{\partial}{\partial \theta_j} \left(\E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right] \right)\\
     &=&
    \lambda_j - \E_\gamma \left[\frac{\partial}{\partial \theta_j}  \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right] \\
    \lambda^{*}_j &=& \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right] \label{logsumexp_probaility}.
\end{eqnarray}

Therefore, the convex conjugate of $f(\theta)$ takes the following values
\begin{equation}\label{conjugate_cases_logsumexp}
    f^{*}\left(\lambda\right) =
        \begin{cases}
            \sum_{i=1}^{d} p_i \theta_i  - \E_\gamma \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right]&\quad\text{if } \lambda = \lambda^{*}\\
            \infty &\quad\text{otherwise}
        \end{cases},
\end{equation}
and its domain $dom f^*(\lambda) = \{\lambda_j^*, j=1, \dots ,d\}$ are probabilities.

Then, since $\partial f(\theta)$ is a probability and the function $f(\theta)$ (Equation \ref{f_theta_logsumexp_perturbed}) is a closed proper convex function on $\R^d$ (Corollary \ref{logsumexp_properties}), the same proof as in the expected max with smooth unbounded perturbations can be applied for the probabilities of the perturbed maximizer (Theorem \ref{theorem_unbounded_smooth_perturb}).  
\end{proof}

Note - For an unperturbed function $f(\theta) = \log (\sum_{i=1}^{d} e^{\theta_i})$, the convex conjugate (Equation \ref{conjugate_cases_logsumexp}) is the negative Shannon entropy
\begin{eqnarray}    
    f^{*}\left(\lambda \right) &=& \sum_{i=1}^{d} p_i \theta_i  - \log (\sum_{i=1}^{d} e^{\theta_i}) \\
    &=& \sum_{i=1}^{d} p_i \left(\theta_i  - \log (\sum_{i=1}^{d} e^{\theta_i}) \right) \\
    &=& \sum_{i=1}^{d} p_i log(p_i)
\end{eqnarray}

\begin{corollary}\label{logsumexp_properties}
$f(\theta)$ (Equation \ref{f_theta_logsumexp_perturbed}) is a closed proper convex function on $R^d$. 
\end{corollary}

\begin{proof}
    \begin{enumerate}
        \item The derivatives of $f(\theta)$ are defined at every point on $\R^d$, therefore $f(\theta)$ is a continuous function. By definition \ref{def:continuous-functions} it is a closed function. 
        \item $f(\theta)$ is convex (Corollary \ref{g_logsumexp_strictconvex} and alternatively Corollary \ref{cor:expectedlogsumexpconvexity}).
        \item  $-\infty \notin dom f(\theta)$,  hence $f(\theta)> -\infty , \forall \theta \in \R^d$ and $f(\theta)$ is a closed proper function by definition  \ref{def:proper-convex- function}.
    \end{enumerate}
\end{proof}

\begin{corollary}
    The probability $\partial f(\theta)$ is a single-valued mapping. 
\end{corollary}

\begin{proof}
    $f(\theta)$ is an essentially smooth and closed proper convex function (Corollary \ref{logsumexp_properties}), therefore Theorem 26.1 \cite{rockafellar-1970a} applies.
\end{proof}

\begin{corollary}\label{logsumexp_stricyconvexitycondition}
    $f(\theta) = \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i})$ 
    is not strictly convex (therefore, a $\nabla f(\theta)$ is not a one-to-one mapping) .
\end{corollary}
\begin{proof}\label{logsumexp_convexityproof1}
    Intuition - Consider the case when $\theta_1 = \theta_2 = \dots = \theta_d=c$. Then $f(\theta) = \log(\sum_{i=1}^d e^{c}) = c+ \log(d)$. The function is affine along this line, so it is not strictly convex. In fact, it is affine along any line of the form  $f(\theta) = c\vec{1}+b$, where $b$ is constant.

    The derivative of $f(\theta)$ is the softmax vector,
    \begin{equation}
        \nabla f(\theta) = g = \frac{1}{\sum_{i=1}^{d} \exp^{\theta_i}}\begin{pmatrix}\exp^{\theta_1} \\ \vdots \\ \exp^{\theta_d} \end{pmatrix},
    \end{equation}
        \begin{equation}
        g_i = \frac{\exp^{\theta_i}}{\sum_{i=1}^{d} \exp^{\theta_i}}. 
    \end{equation}
    Then, $g\succ 0 $ and  $\vec{1}^T g = 1$ and the Hessian $\nabla^2 f(\theta) = diag(g)-gg^T$.

    For $v \in \R^d$ we have that $v^T \nabla^2 f(\theta) v \geq 0 $ since
    \begin{eqnarray}
    v^T \nabla^2 f(\theta) v  &\geq& 0 \\
    v^T diag(g) v &\geq& v^T gg^T v \\
    \sum_{i=1}^{d}(\frac{\exp^{\theta_i}}{\sum_{j=1}^{d} \exp^{\theta_j}})v_i^2 &\geq& \left( \sum_{i=1}^{d} v_i \frac{\exp^{\theta_i}}{\sum_{j=1}^{d} \exp^{\theta_j}} \right)^2 \\
    \E_g \left[ v^2 \right] &\geq&  (\E_g \left[ v \right])^2 \label{logsumexp_convexity} .
    \end{eqnarray}

    The last inequality holds from Jensen's inequality for the convex function $v^2$. Also, since $var(v) = \E \left[ v^2 \right]- (\E \left[ v \right])^2 \geq 0$. 
    
    
    An alternative way to show that $v^T \nabla^2 f(\theta) v \geq 0 $ :
    \begin{eqnarray}
    v^T \nabla^2 f(\theta) v  &\geq& 0 \\
    v^T diag(g) v &\geq& v^T gg^T v \\
    \sum_{i=1}^{d}(\frac{\exp^{\theta_i}}{\sum_{j=1}^{d} \exp^{\theta_j}})v_i^2 &\geq& \left( \sum_{i=1}^{d} v_i \frac{\exp^{\theta_i}}{\sum_{j=1}^{d} \exp^{\theta_j}} \right)^2 \label{logsumexp_convexity_alternative}\\
    \left(\sum_{i=1}^{d}\exp^{\theta_i} v_i^2\right) \left({\sum_{j=1}^{d} \exp^{\theta_j}}\right) &\geq& \left(\sum_{i=1}^{d} v_i \exp^{\theta_i}\right)^2
    \end{eqnarray}

    which holds by Cauchy–Schwarz inequality $  \langle a,a \rangle  \langle b,b \rangle \geq | \langle a,b \rangle |^2 $
    for $a = \begin{pmatrix} \sqrt{\exp^{\theta_1}} \\ \vdots \\ \sqrt{\exp^{\theta_d}} \end{pmatrix}, b = \begin{pmatrix} v_1\sqrt{\exp^{\theta_1}} \\ \vdots \\ v_d\sqrt{\exp^{\theta_d}} \end{pmatrix}$. Equality is obtained when $a$ and $b$ are linearly dependent.    

    When $v = \vec{1}$, Equation \ref{logsumexp_convexity} (alternatively, \ref{logsumexp_convexity_alternative}) holds with equality, i.e., $\vec{1}^T \nabla^2 f(\theta) \vec{1} = 0 $, confirming that $f(\theta)$ is affine along the directions $v = \alpha \vec{1}$ and is convex. For any $v \neq \alpha\vec{1}$, $v^T \nabla^2 f(\theta) v > 0 $, $f(\theta)$ is strictly convex. $\nabla^2 f(\theta)$
    is a rank-1 modification of a positive definite matrix $ diag(\left[g \right)$, then $rank(\nabla^2 f(\theta)))=d-1$. Therefore, $v = \alpha \vec{1}$ 
    are the only vectors for which $\nabla^2 f(\theta))=0$. Thus $f(\theta)$ is strictly convex along any other directions.
\end{proof}


\begin{proof}
    An alternative proof that $f(\theta)$ is convex is based on the high dimensional convexity (Definition \ref{def:highdim_convexity}).
    Consider $h(t) =  f(\theta + tv) = \log (\sum_{i=1}^d \exp^{\theta_i + v_it}) $ for fixed $(\theta,v)$.
    The derivatives of $h(t)$
    \begin{eqnarray}
        h'(t) &=& \langle \nabla f(\theta + tv) , v \rangle\\
        h'(0) &=& \langle \nabla f(\theta) , v \rangle \\
        h''(t) &=& v^T \nabla^2 f(\theta + tv) v. \\
        h''(0) &=& v^T \nabla^2 f(\theta) v.
\textbf{}
    \end{eqnarray}

when \begin{equation}
        \nabla f(\theta + tv) = \frac{1}{\sum_{i=1}^{d} \exp^{\theta_i+v_it}}\begin{pmatrix}\exp^{\theta_1+v_1t} \\ \vdots \\ \exp^{\theta_d+v_dt} \end{pmatrix},
    \end{equation}
        \begin{equation}
        g_j = \frac{\exp^{\theta_j+v_jt}}{\sum_{i=1}^{d} \exp^{\theta_i+v_jt}}. 
    \end{equation}
\begin{eqnarray}
    \partial_k \partial_j f(\theta) &=&
    \frac{- (\exp^{\theta_j+v_jt})(\exp^{\theta_k+v_kt})}{(\sum_{i=1}^{d} \exp^{\theta_i+v_it} )^2}  = -g_jg_k\\ 
    \partial_j \partial_j g(\theta) &=&
    \frac{\exp^{\theta_j+v_jt}(\sum_{i=1}^{d} \exp^{\theta_i+v_it} ) - \exp^{\theta_j+v_jt} \exp^{\theta_j+v_jt} } {(\sum_{i=1}^{d} \exp^{\theta_i+v_it} )^2} =g_j(1-g_j)
\end{eqnarray}

Then, $g \succ 0 $ and  $\vec{1}^T g = 1$ and the Hessian $\nabla^2 f(\theta+vt) = diag(g)-gg^T$.
For the same arguments as in Proof \ref{logsumexp_convexityproof1}, for all $v= \R^d$, 
  $\partial^2 g(t) = v^T \partial^2 f(\theta + tv)  v \geq 0 $, which proves that $f(\theta)$ is convex and strictly convex for any $v\neq \alpha \vec{1}$. 
\end{proof}

\begin{corollary}\label{minimal_rep_holder_logsumexp}
    Let $\theta \in \R^d$. The representation is minimal (Definition \ref{def:minimal_representation}) if the log-sum-exp $f(\theta) = \log (\sum_{i=1}^{d} e^{\theta_i})$ is strictly convex.
\end{corollary}
\begin{proof}



Denote $e^{\theta_i} = u_i$ and  $e^{\theta'_i} = v_i$. Then for $\lambda \in [0,1]$
\begin{eqnarray}
    f(\lambda \theta + (1- \lambda)\theta' )&=& \log(\sum_{i=1}^{d} e^{\lambda \theta_i +(1- \lambda)\theta_i' }) \\
    &=& \log (\sum_{i=1}^{d}u_i^\lambda v_i^{1-\lambda)}) \label{log_sum_eq_dim}.
\end{eqnarray} 
From Hölder's inequality, it holds that for $p, q > 1$ 

\begin{equation}
    \sum_{i=1}^{n} x_iy_i \leq (\sum_{i=1}^{n}|x_i|^p)^{1/p} (\sum_{i=1}^{n}|y_i|^q)^{1/q},
\end{equation}
when $1/p +1/q = 1$. Hölder's inequality holds with equality if with equality when $|y_i| = c |x_i|^{p-1}, \forall i$.

Applying Hölder's inequality to Equation \ref{log_sum_eq_dim} with $1/p= \lambda$ and $1/q = 1-\lambda$ (indeed, for $\lambda \in [0,1]$, it holds that $p \in [1,\infty]$)
\begin{eqnarray}
   \log (\sum_{i=1}^{d}u_i^\lambda v_i^{1-\lambda)})  &\leq & \log\left((\sum_{i=1}^{d} u_i^{\lambda \frac{1}{\lambda}})^\lambda (\sum_{i=1}^{d}v_i^{(1-\lambda) \frac{1}{1-\lambda}})^{1-\lambda} \right) \\ &=&  \lambda \log(\sum_{i=1}^{d}u_i) + (1-\lambda) \log(\sum_{i=1}^{d} v_i)
   \\ &=&  \lambda f(\theta)  +(1-\lambda) f(\theta')   . 
\end{eqnarray} 
Therefore,  we showed that 
\begin{equation}\label{eq:convex_f_holder1}
f(\lambda \theta +(1- \lambda)\theta' ) \leq \lambda f(\theta)  +(1-\lambda) f(\theta'),
\end{equation} proving that $f(\theta)$ is convex.

Hölder's inequality holds with equality and  $f(\theta)$ is convex when $|y_i| = c |x_i|^{p-1}, \forall i$, $e^{\theta_i} = u_i$ and  $e^{\theta'_i} = v_i$, $x_i = u_i^{\lambda}$, $y_i = v_i^{1-\lambda}$, :
\begin{eqnarray}
    e^{(1-\lambda) \theta'_i} &=& c e^{\lambda \theta_i (\frac{1}{\lambda}-1)}\\
    (1-\lambda)\theta'_i  &=& \log(c)+ \lambda\theta_i(\frac{1}{\lambda}-1) \\
    (1-\lambda)\theta'_i  &=& \log(c)+ (1-\lambda)\theta_i \\
    \theta'_i  &=& \frac{\log(c)}{1-\lambda} +\theta_i
    \label{eq:convex_f_holder}
\end{eqnarray} 
in which case $\theta$ and $\theta'$ have a linear constraint. Therefore, the representation is overcomplete since there exists some $\alpha \in \R^2, \alpha \neq 0$ such that $\alpha_1 \theta  + \alpha_2 \theta' = const$.

If Hölder's inequality is strict, $f(\theta)$ is strictly convex, and the representation is minimal.


\textbf{Sanity check}
\begin{enumerate}
\item For $p=2$, $\lambda=0.5$, Equation \ref{eq:convex_f_holder1} reads:
    \begin{eqnarray}
        f(0.5\theta +0.5 \theta') \leq 0.5f(\theta)+0.5f(\theta')\\
        \log(\sum_i e^{0.5\theta_i +0.5\theta'_i }) \leq 0.5\log(\sum_i e^{\theta_i})+ 0.5\log(\sum_i e^{\theta'_i})
    \end{eqnarray}
    Hölder's inequality holds with equality when $|y_i| = c |x_i|^{p-1}, \forall i$. Equation \ref{eq:convex_f_holder} reads:
    \begin{eqnarray}
       \theta' &=& 2\log(c) + \theta
    \end{eqnarray}
    then for $\alpha_1=1$ , $\alpha_2 = -\frac{\theta}{\theta'}=- \frac{\theta}{2\log(c)+\theta}$,
    then 
    \begin{eqnarray}
        \sum_{j=1}^{2} \alpha_j \theta^j &=&  \theta - \frac{\theta}{2\log(c)+\theta} \theta' \\
        &=& \theta - \left(\frac{\theta}{2\log(c)+\theta} \right) \left(2\log(c)+\theta \right)  \\
        &=& 0,
    \end{eqnarray}
confirming that $\sum_{j=1}^{2} \alpha_j \theta^j$ equals a constant and the representation is overcomplete.

\end{enumerate}
\end{proof}





\begin{corollary}
    Let $\theta \in \R^d$ and $\gamma \in \R^d$, $\gamma$ a random variable following a distribution with a smooth pdf $\gamma \sim \mathcal{G}$. The representation of the log-sum-perturbed exp $\E_{\gamma} \left[ f(\theta)\right]  = \E_{\gamma} \left[\log (\sum_{i=1}^{d} e^{\theta_i+ \gamma_i})\right]$  is a.s. minimal and $\E_{\gamma} \left[ f(\theta)\right]$ is strictly convex.
\end{corollary}
\begin{proof}
It follows from Corollary \ref{minimal_rep_holder_logsumexp} that $f(\theta, \gamma)$ is strictly convex a.s. since 
\begin{align}
    P_\gamma \left(\alpha_1(\theta+\gamma) +\alpha_2(\theta'+\gamma') =0 \right) \\ 
    P_\gamma \left( \alpha_1(\theta_1+\gamma_1)+\alpha_1(\theta_2+\gamma_2) + \alpha_2(\theta'_1+\gamma'_1)+\alpha_2(\theta'_2+\gamma'_2) =0 \right) \\
    P_\gamma \left( \alpha_1(\gamma_1+\gamma_2)+\alpha_2(\gamma'_1+\gamma'_2) = -\alpha_1(\theta_1+\theta'_1)-\alpha_2(\theta_1+\theta'_2) \right) \\
    P_\gamma \left( \alpha_1(\gamma_1+\gamma_2)+\alpha_2(\gamma'_1+\gamma'_2) = c \right),
\end{align}
when $-\alpha_1(\theta_1+\theta'_1)-\alpha_2(\theta_1+\theta'_2)$ equals a constant, denoted $c$.

Since $\gamma + \gamma'$ are independent random variables with smooth probability density function,  their sum also has a smooth probability density function. Consequently, the probability that $\sum_{i=1}^d  \alpha_1\gamma_i + \alpha_2 \gamma'_i = c$ is zero, and thus $\P_\gamma\left(\alpha_1(\theta+\gamma) +\alpha_1(\theta'+\gamma') =c \right) = 0$. Hence, $f(\theta, \gamma) $ is a.s. strictly convex and the representation is a.s. minimal.
\end{proof}

\begin{corollary}\label{cor:expectedlogsumexpconvexity}
    $f(\theta) = \E_{\gamma} \left[ \log (\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right]$ 
    is convex along all directions $v= \R^d$,  and strictly convex along any direction $v\neq \alpha \vec{1}$ .
\end{corollary}
\begin{proof}\label{expectedlogsumexpconvexity1}
    
We have:
\begin{eqnarray}
    \partial_j f(\theta) &=& \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right] = \E_\gamma \left[ g_j \right]\\ 
    \partial_k \partial_j f(\theta) &=& \partial_k \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  \\
    &=&  \E_\gamma \left[\partial_k 
    \frac{e^{\theta_j+\gamma_j}}{ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  \\
    &=& \E_\gamma \left[ 
    \frac{- (e^{\theta_j+\gamma_j})(e^{\theta_k+\gamma_k})}{(\sum_{i=1}^{d} e^{\theta_i+\gamma_i} )^2} \right] \\
    &=&   - \E_\gamma \left[g_j g_k  \right]  \\ 
    \partial_j \partial_j f(\theta) &=&
    \E_\gamma \left[\partial_j 
    \frac{e^{\theta_j+\gamma_j}}{ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  \\
    &=& \E_\gamma \left[ 
    \frac{e^{\theta_j+\gamma_j}(\sum_{i=1}^{d} e^{\theta_i+\gamma_i} ) - e^{\theta_j+\gamma_j} e^{\theta_j+\gamma_j} } {(\sum_{i=1}^{d} e^{\theta_i+\gamma_i} )^2} \right] \\
    &=&  \E_\gamma \left[ g_j(1-g_j)  \right]
\end{eqnarray}

    \begin{equation}
        \partial f(\theta) = \E_\gamma \left[ g \right]=  \E_\gamma \left[\begin{pmatrix} g_1 \\ \vdots \\ g_d \end{pmatrix} \right],
    \end{equation}

    Then, $\E_\gamma \left[g\succ 0 \right]$ and  $\vec{1}^T \E_\gamma \left[g \right]= 1$ (Equation \ref{log_sum_exp_conjgate_prob}). 
    The Hessian $\nabla^2 f(\theta) = diag(\E_\gamma \left[g \right])-\E_\gamma \left[gg^T\right]$.


    For $v \in \R^d$ we have that $v^T \nabla^2 f(\theta) v \geq 0 $ since
    \begin{eqnarray}
    v^T \nabla^2 f(\theta) v  &\geq& 0 \\
    v^T diag(\E_\gamma \left[g \right])v &\geq& v^T \E_\gamma \left[gg^T \right] v \\
    \sum_{i=1}^{d} \E_\gamma \left[\frac{\exp^{\theta_i+ \gamma_i}}{\sum_{j=1}^{d} \exp^{\theta_j + \gamma_j}} \right] v_i^2 &\geq& \left( \sum_{i=1}^{d} v_i  \E_\gamma \left[ \frac{\exp^{\theta_i+ \gamma_i}}{\sum_{j=1}^{d} \exp^{\theta_j+ \gamma_j}} \right] \right)^2  \label{expectedlogsumexp_convexity}\\
    \E_{p_\gamma(\theta)} \left[ v^2 \right] &\geq&  (\E_{p_\gamma(\theta)}  \left[ v \right])^2 \label{expectedlogsumexp_convexity_c} .
    \end{eqnarray}

Equation  \ref{expectedlogsumexp_convexity}
holds with equality for $v = \alpha \vec{1}$ since  $\vec{1}^T \E_\gamma \left[g \right]= 1$ (Equation \ref{log_sum_exp_conjgate_prob}). For any other $v \neq  \alpha \vec{1}$, equation  \ref{expectedlogsumexp_convexity}
holds due to the convexity of the squared function $v^2$ (Equation \ref{expectedlogsumexp_convexity_c}), where we denoted $p_\gamma(\theta_i) =\E_\gamma \left[\frac{\exp^{\theta_i+ \gamma_i}}{\sum_{j=1}^{d} \exp^{\theta_j + \gamma_j}} \right]  $.\hedda{need to add a proof that  $v = \alpha \vec{1}$ 
 are the only vectors for which $\nabla^2 f(\theta))=0$} . Specifically, is the rank of $\E_\gamma \left[gg^T\right]$ 1?.

\end{proof}



\begin{corollary}\label{g_logsumexp_strictconvex}
    (An alternative formulation of Corollary \ref{cor:expectedlogsumexpconvexity}). Consider 
    \begin{equation}\label{def:logsumexpexteneded}
        g(\theta) =f(0,\theta) =  \E_\gamma \left[log(1+\sum_{i=1}^{d} e^{\theta_i+\gamma_i}))\right].
    \end{equation} Meaning, $g(\theta): \R^{d+1} \rightarrow \R$ is the expected log-sum-exp function with an added element $\theta_0 = 0$. 
    Then, $g(\theta)$ is strictly convex.
\end{corollary}
\begin{proof}
This proof follows the non-perturbed proof in Appendix A in \cite{nielsen2018monte}.

$g(\theta)$ is twice continuously differentiable, it suffices to prove that $\nabla^2 g(\theta) \succ 0$.
    
We have:
\begin{eqnarray}
    \partial_j g(\theta) &=& \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right] \\ 
    \partial_k \partial_j g(\theta) &=& \partial_k \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]   =  \E_\gamma \left[\partial_k 
    \frac{e^{\theta_j+\gamma_j}}{1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  = \E_\gamma \left[ 
    \frac{- (e^{\theta_j+\gamma_j})(e^{\theta_k+\gamma_k})}{(1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i} )^2} \right] \\ 
    \partial_j \partial_j g(\theta) &=&
    \E_\gamma \left[\partial_j 
    \frac{e^{\theta_j+\gamma_j}}{1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right]  = \E_\gamma \left[ 
    \frac{e^{\theta_j+\gamma_j}(1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i} ) - e^{\theta_j+\gamma_j} e^{\theta_j+\gamma_j} } {(1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i} )^2} \right] 
\end{eqnarray}

The Hessian $\nabla^2 g(\theta)$ is a strictly diagonally dominant matrix since:

\begin{eqnarray}
    \E_\gamma \left[ 
    e^{\theta_j+\gamma_j}(1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i} )  \right]  &=& \E_\gamma \left[ 
    e^{\theta_j+\gamma_j} + e^{\theta_j+\gamma_j}\sum_{i=1}^{d} e^{\theta_i+\gamma_i}   \right] \\
    &>& \E_\gamma \left[ \sum_{k \neq j} |- e^{\theta_j+\gamma_j} e^{\theta_k+\gamma_k} | \right] \\
    &=&  \E_\gamma \left[ e^{\theta_j+\gamma_j} \sum_{k \neq j} e^{\theta_k+\gamma_k} \right] .
\end{eqnarray}

Further, the Hessian has real positive diagonal entries.
Following Gershgorin circle theorem \cite{Varga2004GersgorinAH} we bound the spectrum
of a square matrix: The eigenvalues of the Hessian matrix are thus real and fall inside the disks of centers
$\E_\gamma \left[e^{\theta_j+\gamma_j}(1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i} )  \right] $ and radius $ \E_\gamma \left[ e^{\theta_j+\gamma_j} \sum_{k \neq j} e^{\theta_k+\gamma_k} \right]$. It follows (since the Hessian is strictly diagonally dominant matrix)  that all eigenvalues are positive. Further, since the Hessian is symmetric, it is
positive definite.

\end{proof}

\begin{definition}
    The Gershgorin circle theorem \cite{Varga2004GersgorinAH}:
    Let $A$ be an $n\times n$ matrix with entries in $\mathcal{C}$.
    For each $i$, let $D_i$ be the disc:
    \begin{equation}
        D_i = \{z\in \mathcal{C} : |z-A_{ii}| \leq \sum_{j\neq i} |Aij| \}
    \end{equation}
then the eigenvalues of $A$ lie in $D_1 \cup D_2 \cdots \cup D_n$. 

\textbf{Intuition- } As we draw the discs $D_i, i= 1,...,d+1$ we realize that for a strictly diagonally dominant matrix the union of discs can not include the origin, therefore all eigenvalues are positive.
\end{definition}

{\color{red}{STRICTLY CONVEX IN THE QUOTIENT SPACE $\R^d / 1$}}
\begin{definition}QUOTIENT SPACE: 
Let $V$ be a vector space over a field 
$\mathbb {K}$, and let $N$ be a subspace of 
$V$. We define an equivalence relation 
$\sim$ on $V$ by stating that
\begin{equation}\label{def:QUOTIENTSPACE_relation}
    x\sim y \quad \text{if} \quad {\displaystyle x-y\in N}
\end{equation}. 
That is, $x$ is related to $y$ if one can be obtained from the other by adding an element of $N$.

From this definition, one can deduce that any element of $N$ is related to the zero vector; more precisely, all the vectors in 
$N$ get mapped into the equivalence class of the zero vector.

The equivalence class $\sim$ or, in this case, the coset – of $x$ is often denoted
\begin{equation}
 [x] =x+N
\end{equation}
since it is given by
\begin{equation}\label{def:coset}
[x]=\{x+n:n\in N\}.
\end{equation}
The quotient space ${\displaystyle V/N}$ is then defined as ${\displaystyle V/_{\sim }}$, the set of all equivalence classes induced by $\sim$ on $V$.
\end{definition}

\textbf{example 1}
Let $V = \R^2 = \{(x,y): x,y \in \R \}$, and $N = \{(x,0): x\in \R \}$ the $x$-axis in the 2-d plane.
Then, by Equation \ref{def:QUOTIENTSPACE_relation}, 
\begin{equation}
    (x,y) \sim (x',y') \quad \text{if} \quad {\displaystyle (x,y)-(x',y') \in N}
\end{equation}
therefore, $(x,y) \sim (x',y')$ if $y=y'$.
So the coset (Equation \ref{def:coset}) of an $(x,y)$,
\begin{equation}\label{def:coset}
[(x,y)]=\{(x,y)+n:n\in N\}, 
\end{equation}
are all points that have the given $y$-coordinate. 

All cosets are all lines (affine subspace of $V$) parallel to $N$. 

\begin{figure}[ht!]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/QUOTIENTSPACE_relation_ex1.jpg}
\end{subfigure}
\caption{Illustration of coset, example 1.}
\label{fig:QUOTIENTSPACE_relation_example1}
\end{figure}

\textbf{example 2}
Let $V = \R^2 = \{(x,y): x,y \in \R \}$, and $N = \{(1,1) \}$ the vector $\vec{1}$. 
By Equation \ref{def:QUOTIENTSPACE_relation}, 
\begin{equation}
    (x,y) \sim (x',y') \quad \text{if} \quad {\displaystyle (x,y)-(x',y') \in N}
\end{equation}
therefore, $(x,y) \sim (x',y')$ if $x-x'=1$ and $y-y'=1$.
Meaning, $V/N$ is the vector space of cosets of $V$, i.e. all lines (affine subspace of $V$) parallel to $N$. 
\begin{figure}[ht!]
\centering
\begin{subfigure}{.45\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/QUOTIENTSPACE_relation_ex2.jpg}
\end{subfigure}
\caption{Illustration of the closet of a given (x,y) , example 2.}
\label{fig:QUOTIENTSPACE_relation_example2}
\end{figure}

To generalize, if $V = \R^d$, and $N =\vec{1}^d $, then $V/N$ is the vector space of all d-dimensional planes parallel to $N$.


\begin{corollary}
    Consider $g(\theta) =f(0,\theta) =  \E_\gamma \left[log(1+\sum_{i=1}^{d} e^{\theta_i+\gamma_i}))\right]$. Meaning, $g(\theta): \R^{d+1} \rightarrow \R$ is the expected log-sum-exp function with an added element $\theta_0 = 0$. 
    Then, $\partial g(\theta)$ is a one-to-one probability mapping.
\end{corollary}

\begin{proof}
    $g(\theta)$ is an essentially smooth and a closed proper convex function (Corollary \ref{logsumexp_properties}). Since $g(\theta)$ is also strictly convex \cite{nielsen2018monte} (also in Corollary \ref{g_logsumexp_strictconvex}),  Corollary 26.3.1 \cite{rockafellar-1970a} applies and $\partial g(\theta)$ is a one-to-one mapping. Further,the derivatives of $g(\theta)$,
    \begin{equation}
        \frac{\partial g(\theta)}{\partial \theta_j} = \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=1}^{d} e^{\theta_i+\gamma_i}} \right],
    \end{equation}
    are probabilities (non-negative and sum to one  (similar arguments as in Equations \ref{log_sum_exp_conjgate_prob}, \ref{log_sum_exp_conjgate_prob_nonneg}).    
\end{proof}

\begin{corollary}\label{cor: g_domain}It holds that 
domain $g^*$ are probabilities, $dom g^* \subseteq \Delta$.
\end{corollary}
\begin{proof}
    
The convex conjugate of $g(\theta)$ is
\begin{equation}
    g^{*}\left(\lambda\right):=\sup _{\theta\in \R^{d+1}} \{\langle \theta,\lambda \rangle - \E_\gamma \left[ \log (1+\sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right] \}.
\end{equation}
Derivative w.r.t. $\theta_j$ and apply Leibniz's integral rule for differentiation under the integral sign,
\begin{eqnarray}
    \frac{\partial g^{*}}{\partial \theta_j} &=&
    \lambda_j - \E_\gamma \left[\frac{\partial}{\partial \theta_j}  \log (\sum_{i=0}^{d} e^{\theta_i+\gamma_i}) \right] \\
    \lambda^{*}_j &=& \E_\gamma \left[\frac{e^{\theta_j+\gamma_j}}{\sum_{i=0}^{d} e^{\theta_i+\gamma_i}} \right] \label{logsumexp_strict_probaility}.
\end{eqnarray}
Therefore, the convex conjugate of $g(\theta)$ takes the following values
\begin{equation}\label{conjugate_cases_logsumexp_strict}
    g^{*}\left(\lambda\right) =
        \begin{cases}
            \sum_{i=0}^{d} p_i \theta_i  - \E_\gamma \left[ \log (1+ \sum_{i=1}^{d} e^{\theta_i+\gamma_i}) \right]&\quad\text{if } \lambda = \lambda^{*}\\
            \infty &\quad\text{otherwise}
        \end{cases},
\end{equation}

and its domain $dom g^*(\lambda) = \{\lambda_j^*, j=0, \dots ,d\}$ are probabilities (similar arguments as in Equations \ref{log_sum_exp_conjgate_prob}, \ref{log_sum_exp_conjgate_prob_nonneg}).
\end{proof}

\begin{theorem}
The range of probabilities $\text{range } \partial g(\theta)$ differs very little from the simplex 
    \begin{equation}
        ri( \Delta^d) \subset \text{range }  p_\gamma  \subset \Delta^d.
    \end{equation}
\end{theorem}

\begin{proof}
Following the proof arguments of Theorem \ref{theorem_unbounded_smooth_perturb} requires showing
that $ \text{range }  \partial g \subseteq \Delta$ and that $ri (\Delta) \subseteq  ri (dom g^*)$.

First, it holds that $dom g^* \subseteq \Delta^d$ (Corollary \ref{cor: g_domain}). Since  $ \text{range } \partial g \subset dom g^*$   (Equation \ref{rockafellar_rangedf}), it holds also that  $\text{range }  \partial g  \subseteq \Delta^d$.


The proof follows by showing that  $ri(\Delta^d) \subseteq ri (dom g^*)$. Consider $\theta^0_n = (0,n, \dots, n)$, $\theta_n \in \R^{d+1}$, a vector of all $n$, except its value in the $0^{th}$ position is fixed at $0$. Then, it holds that $\partial g(\theta^0_n)  \in \Delta^{d+1}$ and also $\partial g(\theta^0_n) \in dom f^*$, since we proved that $\text{range } \partial g \subset \text{dom}  g^* \subseteq \Delta^d$. 
The sequence $\left( \partial g(\theta^0_n)\right)_{n_0}^{-\infty}$ is a monotonic and bounded sequence of real numbers, then by the monotone convergence theorem its limit exists.
Hence, the derivative of $g(\theta^0_n)$ approaches an extreme point of the probability simplex as $n \rightarrow -\infty$, since
\begin{eqnarray}\label{limit_prob_g}
    \lim_{n \rightarrow -\infty} \partial g(\theta^0_n) &=& \lim_{n \rightarrow -\infty} (\frac{\partial g(\theta^0_n)}{\partial \theta^0},\dots, \frac{\partial g(\theta^0_n)}{\partial \theta^i},\dots, \frac{\partial g(\theta^0_n)}{\partial \theta^d}) \nonumber  \\ 
    &=& (1,0,\dots, 0) . 
\end{eqnarray}
Therefore, it holds that it is a point in the closure of the $dom  g^*$, $\lim_{n \rightarrow -\infty} \partial g(\theta^0_n) \in cl(dom  g^*)$.
The proof follows with the arguments in Theorem \ref{theorem_unbounded_smooth_perturb} by considering the $\text{range } \partial g(\theta^0_n) \cup \text{range } \partial g(\theta^i_n)$ for $i=1, \dots d$.
\end{proof}

==> sections/Misc/Fisher___Tippett___Gnedenko.tex <==
\section{Fisher-Tippett-Gnedenko Theorem}
\label{Fisher–Tippett–Gnedenko}


The Fisher–Tippett–Gnedenko Theorem (also the Fisher–Tippett theorem or the extreme value theorem) is a general result in extreme value theory regarding asymptotic distribution of extreme order statistics. The maximum of a sample of iid random variables after proper renormalization can only converge in distribution to one of 3 possible distributions, the Gumbel distribution, the Fréchet distribution, or the Weibull distribution. 

Let $X_{1},X_{2},\ldots ,X_{n}$ be a sequence of independent and identically distributed random variables with cumulative distribution function $F$. Suppose that there exist two sequences of real numbers $a_{n}>0$ and $b_{n} \in \mathbb{R}$ such that the following limits converge to a non-degenerate distribution function:
\begin{equation}
    \lim _{n \to \infty } P\left({\frac {\max\{X_{1},\dots ,X_{n}\}-b_{n}}{a_{n}}}\leq x\right)=G(x),
\end{equation}
or equivalently:
\begin{equation}
    \lim _{n\to \infty }F^{n}\left(a_{n}x+b_{n}\right)=G(x).
\end{equation}
In such circumstances, the limit distribution $G$ belongs to either the Gumbel, the Fréchet, or the Weibull family.
In other words, if the limit above converges, then up to a linear change of coordinates $G(x)$ will assume the form:
\begin{equation}
    G_{\gamma }(x)=\exp \left(-(1+\gamma \,x)^{-1/\gamma }\right),\;\;1+\gamma \,x>0
\end{equation}
or else
\begin{equation}
        G_{0}(x)=\exp \left(-\exp(-x)\right)
\end{equation}
for some parameter $\gamma$. This is the cumulative distribution function of the generalized extreme value distribution (GEV) with extreme value index $\gamma$. The GEV distribution groups the Gumbel, Fréchet, and Weibull distributions into one. Note that the second formula (the Gumbel distribution) is the limit of the first as $\gamma$  goes to zero.

\subsection{Convergence of the extreme value for the standard normal distribution}

Let $X_{1},X_{2},\ldots ,X_{n}$ be a sequence of 
be i.i.d. random variables with cumulative distribution function of the Standard Normal distribution, 
\begin{equation}\label{normal_cdf}
    F(x)=\frac {1}{\sqrt {2\pi }}\int _{-\infty }^{x}e^{-t^{2}/2}\,dt .
\end{equation}

We have
\begin{equation}
\ln F(x)\sim -{\frac {\exp(-x^{2}/2)}{{\sqrt {2\pi }}x}}
\end{equation}
and
\begin{equation}
\ln F(x)^{n}=n\ln F(x)\sim -{\frac {n\exp(-x^{2}/2)}{{\sqrt {2\pi }}x}}.
\end{equation}
Thus we have
\begin{equation}
    F(x)^{n}\approx \exp \left(-{\frac {n\exp(-x^{2}/2)}{{\sqrt {2\pi }}x}}\right).
\end{equation}
If we define $c_{n}$ as the value that satisfies
\begin{equation}
    \frac {n\exp(-c_{n}^{2}/2)}{{\sqrt {2\pi }}c_{n}}=1    
\end{equation}
then around $x=c_{n}$
\begin{equation}
    {\frac {n\exp(-x^{2}/2)}{{\sqrt {2\pi }}x}}\approx \exp(c_{n}(c_{n}-x)).
\end{equation}
As n increases, this becomes a good approximation for a wider and wider range of $(c_{n}-x)$ so letting $u=c_{n}$ we find that
\begin{equation}
     \lim _{n\to \infty }F(u/c_{n}+c_{n})^{n}=\exp(-\exp(-u))=G_{0}(u).
\end{equation}
Equivalently,
\begin{equation}
    \lim _{n\to \infty }P{\Bigl (}{\frac {\max\{X_{1},\ldots ,X_{n}\}-c_{n}}{1/c_{n}}}\leq u{\Bigr )}=\exp(-\exp(-u))=G_{0}(u).
\end{equation}


\section{The Gaussian-Max trick}

Let $\gamma = \{\gamma_i: i = 1,...,n  \}$ be a collection of i.i.d. normal random
variables with cumulative distribution function F (Equation \ref{normal_cdf}) and let $\theta = \{\theta_i : i = 1,...,n   \}$ be the collection of potential functions for each configuration $i$. Then, 
\begin{eqnarray}
   \lim_{n \rightarrow \infty} P_\gamma( \frac{\max_{i} \{\theta_i+\gamma_i\}- b_n}{a_n} \leq x )  =
\lim_{n \rightarrow \infty} P_\gamma( \forall_i \frac{ \theta_i+\gamma_i- b_n}{a_n} \leq x )  \\
= \lim_{n \rightarrow \infty} P_\gamma( \forall_i \gamma_i \leq a_n x + b_n -\theta_i)  \\
= \lim_{n \rightarrow \infty} \prod_i F(a_nx+b_n-\theta_i)  \\
\approx = \lim_{n \rightarrow \infty}  \prod_i  \exp \left(-{\frac { \exp(-(a_n x + b_n -\theta_i)^{2}/2)}{{\sqrt {2\pi }}(a_n x + b_n -\theta_i)}}\right) \\
\text{by a change of parameter } \hat \theta_i = b_n- \theta_i  \nonumber \\ 
\approx =\lim_{n \rightarrow \infty}  \prod_i  \exp \left(-{\frac { \exp(-(a_n x + \hat \theta_i)^{2}/2)}{{\sqrt {2\pi }}(a_n x + \hat \theta_i)}}\right)\\
\approx =\lim_{n \rightarrow \infty}  \prod_i  \exp \left(-{\frac { \exp(-(a_n^2 x^2 + 2 a_n \hat \theta_i  x + \hat \theta_i^2)/2)}{{\sqrt {2\pi }}(a_n x + \hat \theta_i)}}\right)
\end{eqnarray}



==> summary_probabilities_perturbation_models.tex <==
\section{Summary- Probabilities of perturbation models}\label{summary_probabilities_perturbation_models}

\begin{table}[h]
\begin{tabular}{l|ll|ll|}
\cline{2-5}
                                       & \multicolumn{2}{c|}{\textbf{Perturbed Max}} & \multicolumn{2}{c|}{\textbf{Perturbed log-sum-exp}} \\ \hline
\multicolumn{1}{|l|}{Perturbation} &
  \multicolumn{1}{l|}{Single-valued mapping} &
  $\Delta^{d-1}$ &
  \multicolumn{1}{l|}{Single-valued mapping} &
  $\Delta^{d-1}$ \\ \hline
\multicolumn{1}{|l|}{smooth unbounded} & \multicolumn{1}{l|}{yes}      & almost      & \multicolumn{1}{l|}{yes}  & almost      \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}smooth bounded \\ (e.g. uniform)\end{tabular}} &
  \multicolumn{1}{l|}{no} &
  yes &
  \multicolumn{1}{l|}{yes} &
  almost \\ \hline
\multicolumn{1}{|l|}{discrete}         & \multicolumn{1}{l|}{no}       & yes         & \multicolumn{1}{l|}{yes}            & almost           \\ \hline
\end{tabular}
\end{table}
